Batch Reinforcement Learning with a Nonparametric Off-Policy Policy Gradient

Off-policy Reinforcement Learning (RL) holds the promise of better data efficiency as it allows sample reuse and potentially enables safe interaction with the environment. Current off-policy policy gradient methods either suffer from high bias or high variance, delivering often unreliable estimates. The price of inefficiency becomes evident in real-world scenarios such as interaction-driven robot learning, where the success of RL has been rather limited, and a very high sample cost hinders straightforward application. In this paper, we propose a nonparametric Bellman equation, which can be solved in closed form. The solution is differentiable w.r.t the policy parameters and gives access to an estimation of the policy gradient. In this way, we avoid the high variance of importance sampling approaches, and the high bias of semi-gradient methods. We empirically analyze the quality of our gradient estimate against state-of-the-art methods, and show that it outperforms the baselines in terms of sample efficiency on classical control tasks.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> TPAMI-2021 arxiv/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> TPAMI-2021 arxiv/experiments/Cartpole_random.tex <==
\begin{figure}[t]
\begin{centering}
    \centering
    \includegraphics[scale=0.6]{figures/experiments/cartpole_randomwalk_samplesize.pdf}
    \caption[Returns in the Cartpole stabilization environment with randomly sampled data]{\textbf{Returns in the Cartpole stabilization environment with randomly sampled data} This plot compares the return obtained by NOPG and typical on- and off-policy algorithms in the CartPole task, as a function of the number of collected samples. NOPG's performance surpasses other algorithms by at least an order of magnitude. The TRPO and DDPG curves start at $5 \cdot 10^2$ samples because to accelerate training we only evaluate these algorithms after collecting every other $5 \cdot 10^2$ samples. The solid line represents the mean and the shaded area the 95\% confidence interval of 10 runs. The details used in this experiment are presented in \tabref{tab:cartpole_random_configs}.}

    \label{fig:cartpole_random}
\end{centering}
\end{figure}


==> TPAMI-2021 arxiv/experiments/Cartpole_random_configs.tex <==
The following tables show the hyper-parameters used to generate the third plot in Figure~\ref{figure:comparison}.
\begin{center}
    \begin{longtable}{l l}
        \textbf{NOPG} & \\
        \hline
        dataset sizes & $10^2$, $2.5 \cdot 10^2$, $5 \cdot 10^2$, $10^3$, $1.5 \cdot 10^3$, $2.5 \cdot 10^3$,  \\
                      & $3 \cdot 10^3$, $5 \cdot 10^3$, $6 \cdot 10^3$, $8 \cdot 10^3$, $10^4$ \\        
        discount factor $\gamma$ & $0.99$ \\
        state $\vec{h}_{\textrm{factor}}$ & $1.0$ $1.0$ $1.0$  \\
        action $ \vec{h}_{\textrm{factor}}$ & $20.0$ \\
        policy & neural network parameterized by $\bm{\theta}$\\
               & $1$ hidden layer, $50$ units, ReLU activations \\
        policy output & $5 \tanh(f_{\bm{\theta}}(\state))$ (NOGP-D) \\
                      & $\mu = 5 \tanh(f_{\bm{\theta}}(\state))$, $\sigma = \textrm{sigmoid}(g_{\bm{\theta}}(\state))$ (NOGP-S) \\               
        learning rate  & $ 10^{-2}$ with ADAM optimizer \\
        $N_{\pi}^{\textrm{MC}}$ (NOPG-S) & $10$ \\
        $N_{\phi}^{\textrm{MC}}$ & $1$ \\
        $N_{\mu_0}^{\textrm{MC}}$ & $15$ \\
        policy updates & $2 \cdot 10^3$ \\
        \hline
        & \\ & \\
        
        \textbf{SAC} & \\
        \hline
        discount factor $\gamma$ & $0.99$ \\
        rollout steps & $10000$ \\
        actor  & neural network parameterized by $\bm{\theta}_{\textrm{actor}}$\\
        & $1$ hidden layer, $50$ units, ReLU activations \\
        actor output & $5 \tanh(u)$, $u \sim \mathcal{N}(\cdot | \mu = f_{\bm{\theta}_{\textrm{actor}}}(\state), \sigma = g_{\bm{\theta}_{\textrm{actor}}}(\state))$ \\
        actor learning rate & $10^{-3}$ with ADAM optimizer \\
        critic  & neural network parameterized by $\bm{\theta}_{\textrm{critic}}$\\
        & $2$ hidden layers, $50$ units, ReLU activations \\
        critic output & $f_{\bm{\theta}_{\textrm{critic}}}(\state, \action)$ \\
        critic learning rate & $5 \cdot 10^{-3}$ with ADAM optimizer \\        
        max replay size & $5 \cdot 10^5$ \\
        initial replay size & $128$ \\
        batch size & $64$ \\
        soft update & $\tau = 5 \cdot 10^{-3}$ \\
        policy updates & $2.5 \cdot 10^5$ \\
        \hline        
        & \\ & \\    
        
        \textbf{DDPG / TD3} & \\
        \hline
        discount factor $\gamma$ & $0.99$ \\
        rollout steps & $10000$ \\
        actor  & neural network parameterized by $\bm{\theta}_{\textrm{actor}}$\\
               & $1$ hidden layer, $50$ units, ReLU activations \\
        actor output & $5 \tanh(f_{\bm{\theta}_{\textrm{actor}}}(\state))$ \\
        actor learning rate & $10^{-3}$ with ADAM optimizer \\
        critic  & neural network parameterized by $\bm{\theta}_{\textrm{critic}}$\\
                & $1$ hidden layer, $50$ units, ReLU activations \\
        critic output & $f_{\bm{\theta}_{\textrm{critic}}}(\state, \action)$ \\
        critic learning rate & $10^{-2}$ with ADAM optimizer \\        
        soft update & $\tau = 10^{-3}$ \\
        policy updates & $2 \cdot 10^5$ \\
        \hline        
        & \\ & \\ & \\
%        
%        \textbf{DDPG Offline} & \\
%        \hline
%        dataset sizes & $10^2$, $5 \cdot 10^2$, $10^3$, $2 \cdot 10^3$, $3.5 \cdot 10^3$, $5 \cdot 10^3$, \\
%                      & $8 \cdot 10^3$,  $10^4$, $1.5 \cdot 10^4$, $2 \cdot 10^4$, $2.5 \cdot 10^4$ \\        
%        discount factor $\gamma$ & $0.99$ \\
%        actor  & neural network parameterized by $\bm{\theta}_{\textrm{actor}}$\\
%               & $1$ hidden layer, $50$ units, ReLU activations \\
%        actor output & $5 \tanh(f_{\bm{\theta}_{\textrm{actor}}}(\state))$ \\
%        actor learning rate & $10^{-2}$ with ADAM optimizer \\
%        critic  & neural network parameterized by $\bm{\theta}_{\textrm{critic}}$\\
%                & $1$ hidden layer, $50$ units, ReLU activations \\
%        critic output & $f_{\bm{\theta}_{\textrm{critic}}}(\state, \action)$ \\
%        critic learning rate & $10^{-2}$ with ADAM optimizer \\
%        soft update & $\tau = 10^{-3}$ \\
%        policy updates & $2 \cdot 10^3$ \\
%        \hline
%        & \\ & \\

        \textbf{PWIS} & \\
        \hline
        dataset sizes & $10^2$, $5 \cdot 10^2$, $10^3$, $2 \cdot 10^3$, $3.5 \cdot 10^3$, $5 \cdot 10^3$, \\
                      & $8 \cdot 10^3$,  $10^4$, $1.5 \cdot 10^4$, $2 \cdot 10^4$, $2.5 \cdot 10^4$ \\          
        discount factor $\gamma$ & $0.99$ \\
        policy & neural network parameterized by $\bm{\theta}$\\
               & $1$ hidden layer, $50$ units, ReLU activations \\
        policy output & $\mu = 5 \tanh(f_{\bm{\theta}}(\state))$, $\sigma = \textrm{sigmoid}(g_{\bm{\theta}}(\state))$ \\               
        learning rate  & $10^{-3}$ with ADAM optimizer \\
        policy updates & $2 \cdot 10^3$ \\
        \hline
        & \\ & \\ & \\
        
        \textbf{BEAR} & \\
        \hline
        dataset sizes & $10^2$, $2 \cdot 10^2$ $5 \cdot 10^2$, $10^3$, $2 \cdot 10^3$, $5 \cdot 10^3$, \\
        & $10^4$, $2 \cdot 10^4$, $5 \cdot 10^4$, $10^5$ \\          
        discount factor $\gamma$ & $0.99$ \\
        policy & neural network parameterized by $\bm{\theta}$\\
        & $1$ hidden layer, $50$ units, ReLU activations \\
        policy output & $\mu = 5 \tanh(f_{\bm{\theta}}(\state))$, $\sigma = \textrm{sigmoid}(g_{\bm{\theta}}(\state))$ \\               
        learning rate  & $10^{-4}$ \\
        policy updates & $1 \cdot 10^3$ \\
        \hline
        & \\ & \\ & \\
        
        \textbf{BRAC-(dual)} & \\
        \hline
        dataset sizes & $10^2$, $2 \cdot 10^2$ $5 \cdot 10^2$, $10^3$, $2 \cdot 10^3$, $5 \cdot 10^3$, \\
        & $10^4$, $2 \cdot 10^4$, $5 \cdot 10^4$, $10^5$ \\          
        discount factor $\gamma$ & $0.99$ \\
        policy & neural network parameterized by $\bm{\theta}$\\
        & $1$ hidden layer, $50$ units, ReLU activations \\
        policy output & $\mu = 5 \tanh(f_{\bm{\theta}}(\state))$, $\sigma = \textrm{sigmoid}(g_{\bm{\theta}}(\state))$ \\               
        learning rate  & $10^{-3}$ with Adam \\
        policy updates & $5 \cdot 10^4$ \\
        batch size & $\leq 256$ \\
        soft update & $\tau = 5 \cdot 10^{-3}$ \\
        \hline
        & \\ & \\ & \\        

        \textbf{MOPO} & \\
		\hline
		dataset sizes & $10^2$, $2 \cdot 10^2$ $5 \cdot 10^2$, $10^3$, $2 \cdot 10^3$, $5 \cdot 10^3$, \\
		& $10^4$, $2 \cdot 10^4$, $5 \cdot 10^4$, $10^5$ \\          
		discount factor $\gamma$ & $0.99$ \\
		policy & neural network parameterized by $\bm{\theta}$\\
		& $1$ hidden layer, $50$ units, ReLU activations \\
		policy output & $\mu = 2 \tanh(f_{\bm{\theta}}(\state))$, $\sigma = \textrm{sigmoid}(g_{\bm{\theta}}(\state))$ \\               
		learning rate  & $3 \cdot 10^{-4}$ with Adam \\
		number of epochs & $5 \cdot 10^2$ \\
		batch size & $256$ \\
		soft update & $\tau = 5 \cdot 10^{-3}$ \\
		BNN hidden dims & $32$ \\
		BNN max epochs & $100$ \\ 
		BNN ensemble size & $7$ \\
		\hline
		& \\ & \\ & \\
		
		\textbf{MOReL} & \\
		\hline
		dataset sizes & $10^2$, $2 \cdot 10^2$ $5 \cdot 10^2$, $10^3$, $2 \cdot 10^3$, $5 \cdot 10^3$, \\
		& $10^4$, $2 \cdot 10^4$, $5 \cdot 10^4$, $10^5$ \\          
		discount factor $\gamma$ & $0.99$ \\
		policy & neural network parameterized by $\bm{\theta}$\\
		& $1$ hidden layer, $50$ units, ReLU activations \\
		policy output & $\mu = 2 \tanh(f_{\bm{\theta}}(\state))$, $\sigma = \textrm{sigmoid}(g_{\bm{\theta}}(\state))$ \\               
		step size & $0.02$ \\
		number of iterations & $500$ \\
		dynamics hidden dims & $(128, 128)$, ReLU activations \\
		dynamics lr & $0.001$ \\
		dynamics batch-size & $256$ \\	
		dynamics fit-epochs & $25$ \\	
		dynamics num-models & $4$ \\
		\hline        


        \caption[Algorithms configurations for the CartPole random data experiment]{\textbf{Algorithms configurations for the CartPole random data experiment}.}
        \label{tab:cartpole_random_configs}
            
    \end{longtable}
\end{center}




==> TPAMI-2021 arxiv/experiments/Cartpole_real.tex <==
\begin{figure}[t]
\begin{centering}
    \centering
    \includegraphics[scale=0.5]{figures/experiments/cartpole_real.png}
    \caption[Evaluation of a policy optimized with NOPG-S in the real CartPole system]{\textbf{Evaluation of a policy optimized with NOPG-S in the real CartPole system} This stream of figures (left to right, top to bottom ordering) shows the application of a policy learned in simulation with NOPG-S in the real CartPole environment. The policy was trained using 1500 data points from trajectories with actions randomly sampled from a uniform distribution. Although a compliant policy can be learned with less samples, we found its actions alternated between very low and high signals, leading to very rough movements. We noticed that using more samples solved this problem.}
    \label{fig:cartpole_real}
\end{centering}
\end{figure}


==> TPAMI-2021 arxiv/experiments/Environments_schematics.tex <==
\begin{figure}[t]
\begin{centering}
    \begin{subfigure}{0.33\textwidth}
      \centering
      \includegraphics[scale=0.5]{figures/experiments/Pendulum_schematic.pdf}
      \caption{Pendulum}
      \label{fig:pendulum_schematic}
    \end{subfigure}%
    \begin{subfigure}{0.33\textwidth}
      \centering
      \includegraphics[scale=0.5]{figures/experiments/CartPole_schematic.pdf}
      \caption{CartPole}
      \label{fig:cartpole_schematic}
    \end{subfigure}
    \begin{subfigure}{0.33\textwidth}
      \centering
      \includegraphics[scale=0.5]{figures/experiments/MountainCar_schematic.pdf}
      \caption{MountainCar}
      \label{fig:mountaincar_schematic}
    \end{subfigure}    
    
    \caption[Environment schematics]{\textbf{Environment schematics} These figures depict the environments used in the experiments.}
    
    \label{fig:environment_schematics}
\end{centering}
\end{figure}

==> TPAMI-2021 arxiv/experiments/MountainCar_phase_portrait.tex <==
\begin{figure}[t]
\begin{centering}
    \begin{subfigure}{0.5\textwidth}
      \centering
      \includegraphics[scale=0.5]{figures/experiments/MountainCar_V_mu_0.pdf}
      \caption{Before any policy update}
      \label{fig:mountaincar_phase_portrait_a}
    \end{subfigure}%
    \begin{subfigure}{0.5\textwidth}
      \centering
      \includegraphics[scale=0.5]{figures/experiments/MountainCar_V_mu_251.pdf}
      \caption{After 251 policy updates}
      \label{fig:mountaincar_phase_portrait_b}
    \end{subfigure}
    
    \caption[Phase portrait of the value function and state distribution for the MountainCar experiment]{\textbf{Phase portrait of the value function and state distribution for the MountainCar experiment} The plots show the value function and state distribution estimates in the MountainCar environment using NOPG-D. The two leftmost plots show the estimates before any policy update and the rightmost after 251 updates. NOPG-D was trained with 4 trajectories provided by a human demonstrator with the details presented in \tabref{tab:mountaincar_configs}.}
    
    \label{fig:mountaincar_phase_portrait}
\end{centering}
\end{figure}


==> TPAMI-2021 arxiv/experiments/MountainCar_random_configs.tex <==
The dataset ($10$ trajectories) for the experiment in Figure~\ref{figure:mountain} has been generated by a human demonstrator, and is available in the source code provided.

\begin{center}

    \begin{longtable}{l l}
        \textbf{NOPG} & \\
        \hline
        discount factor $\gamma$ & $0.99$ \\
        state $\vec{h}_{\textrm{factor}}$ & $1.0$ $1.0$ \\
        action $ \vec{h}_{\textrm{factor}}$ & $50.0$ \\
        policy & neural network parameterized by $\vec{\theta}$\\
               & $1$ hidden layer, $50$ units, ReLU activations \\
        policy output & $ \tanh(f_{\vec{\theta}}(\state))$ (NOGP-D) \\
                      & $\mu =  \tanh(f_{\vec{\theta}}(\state))$, $\sigma = \textrm{sigmoid}(g_{\vec{\theta}}(\state))$ (NOGP-S) \\               
        learning rate  & $10^{-2}$ with ADAM optimizer \\
        $N_{\pi}^{\textrm{MC}}$ (NOPG-S) & $15$ \\
        $N_{\phi}^{\textrm{MC}}$ & $1$ \\
        $N_{\mu_0}^{\textrm{MC}}$ & $15$ \\
        policy updates & $1.5 \cdot 10^3$ \\
        \hline
        \caption[NOPG configurations for the MountainCar experiment]{\textbf{NOPG configurations for the MountainCar experiment.}}
        \label{tab:mountaincar_configs}
    \end{longtable}
    
\end{center}

==> TPAMI-2021 arxiv/experiments/MountainCar_samplesize.tex <==
\begin{figure}[t]
\begin{centering}
    \centering
    \includegraphics[scale=0.6]{figures/experiments/mountaincar_samplesize.pdf}
    \caption[Returns in the MountainCar environment with varying number of trajectories]{\textbf{Returns in the MountainCar environment with varying number of trajectories} This plot shows the returns obtained by NOPG-D and NOPG-S as a function of the number of trajectories (roughly each trajectory corresponds to 450 samples). The human baseline corresponds to the average return in the human demonstrations and is depicted by the dashed line. The solid line represents the mean and the shaded area the 95\% confidence interval of 10 runs. The details used in this experiment are presented in \tabref{tab:mountaincar_configs}.}
    \label{fig:mountaincar_samplesize}
\end{centering}
\end{figure}


==> TPAMI-2021 arxiv/experiments/MountainCar_trajectory.tex <==
\begin{figure}[t]
\begin{centering}
    \centering
    \includegraphics[scale=0.6]{figures/experiments/MountainCar_trajectories.pdf}
    \caption[Trajectories in the state space of the MountainCar environment]{\textbf{Trajectories in the state space of the MountainCar environment} This figure shows two trajectories from evaluation runs of NOPG-D in the MountainCar environment. Trajectory's $1$ return is $-79$ and trajectory's $2$ is $-139$. The crosses denote the starting states and the circles the final states. The dashed vertical line at $x=-0.45$ depicts the goal state. The policy used was optimized with NOPG-D trained on 4 trajectories provided by a human demonstrator with the details presented in \tabref{tab:mountaincar_configs}.}
    \label{fig:mountaincar_trajectories}
\end{centering}
\end{figure}


==> TPAMI-2021 arxiv/experiments/Pendulum_phase_portrait.tex <==
\begin{figure}[t]
\begin{centering}
    \begin{subfigure}{0.5\textwidth}
      \centering
      \includegraphics[scale=0.5]{figures/experiments/Pendulum_V_mu_0.pdf}
      \caption{Before any policy update}
      \label{fig:pendulum_phase_portrait_a}
    \end{subfigure}%
    \begin{subfigure}{0.5\textwidth}
      \centering
      \includegraphics[scale=0.5]{figures/experiments/Pendulum_V_mu_301.pdf}
      \caption{After 301 policy updates}
      \label{fig:pendulum_phase_portrait_b}
    \end{subfigure}
    
    \caption[Phase portrait of the value function and state distribution for the Pendulum environment]{\textbf{Phase portrait of the value function and state distribution for the Pendulum environment} The plots show the value function and state distribution estimates in the Pendulum environment using NOPG-D, with a uniformly sampled data. The two leftmost plots show the estimates before any policy update and the rightmost after 301 updates. In this experiment, data was collected uniformly from a grid of state-action pairs (30 angles, 30 angular velocities, 2 actions) and NOPG-D trained with the details presented in \tabref{tab:pendulum_uniform_configs}.}
    
    \label{fig:pendulum_phase_portrait}
\end{centering}
\end{figure}


==> TPAMI-2021 arxiv/experiments/Pendulum_random.tex <==
\begin{figure}[t]
\begin{centering}
    \centering
    \includegraphics[scale=0.6]{figures/experiments/pendulum_randomwalk_samplesize.pdf}
    \caption[Returns in the Pendulum environment with randomly sampled data]{\textbf{Returns in the Pendulum environment with randomly sampled data} This plot compares the return obtained by NOPG and typical on- and off-policy algorithms in the Pendulum task, as a function of the number of collected samples. NOPG's performance surpasses other algorithms by at least an order of magnitude. The TRPO and DDPG curves start at $10^3$ samples because to accelerate training we only evaluate these algorithms after collecting every other $10^3$ samples. The solid line represents the mean and the shaded area the 95\% confidence interval of 10 runs. The details used in this experiment are presented in \tabref{tab:pendulum_random_configs}.}
    \label{fig:pendulum_random}
\end{centering}
\end{figure}


==> TPAMI-2021 arxiv/experiments/Pendulum_random_configs.tex <==
The following tables show the hyper-parameters used for generating the second plot starting from the left in Figure~\ref{figure:comparison}
\begin{center}
    \begin{longtable}{l l}
        \textbf{NOPG} & \\
        \hline
        dataset sizes & $10^2$, $5 \cdot 10^2$, $10^3$, $1.5 \cdot 10^3$, $2 \cdot 10^3$, $3 \cdot 10^3$, \\
                      & $5 \cdot 10^3$, $7 \cdot 10^3$, $9 \cdot 10^3$, $10^4$ \\
        discount factor $\gamma$ & $0.99$ \\
        state $\vec{h}_{\textrm{factor}}$ & $1.0$ $1.0$ $1.0$  \\
        action $ \vec{h}_{\textrm{factor}}$ & $25.0$ \\
        policy & neural network parameterized by $\bm{\theta}$\\
               & $1$ hidden layer, $50$ units, ReLU activations \\
        policy output & $2 \tanh(f_{\bm{\theta}}(\state))$ (NOGP-D) \\
                      & $\mu = 2 \tanh(f_{\bm{\theta}}(\state))$, $\sigma = \textrm{sigmoid}(g_{\bm{\theta}}(\state))$ (NOGP-S) \\               
        learning rate  & $10^{-2}$ with ADAM optimizer \\
        $N_{\pi_0}^{\textrm{MC}}$ (NOPG-S) & $10$ \\
        $N_{\phi}^{\textrm{MC}}$ & $1$ \\
        $N_{\mu_0}^{\textrm{MC}}$ & (non applicable) fixed initial state \\        
        policy updates & $2 \cdot 10^3$ \\
        \hline
        & \\ & \\
        
        \textbf{SAC} & \\
		\hline
		discount factor $\gamma$ & $0.99$ \\
		rollout steps & $500$ \\
		actor  & neural network parameterized by $\bm{\theta}_{\textrm{actor}}$\\
		& $1$ hidden layer, $50$ units, ReLU activations \\
		actor output & $2 \tanh(u)$, $u \sim \mathcal{N}(\cdot | \mu = f_{\bm{\theta}_{\textrm{actor}}}(\state), \sigma = g_{\bm{\theta}_{\textrm{actor}}}(\state))$ \\
		actor learning rate & $10^{-3}$ with ADAM optimizer \\
		critic  & neural network parameterized by $\bm{\theta}_{\textrm{critic}}$\\
		& $2$ hidden layers, $50$ units, ReLU activations \\
		critic output & $f_{\bm{\theta}_{\textrm{critic}}}(\state, \action)$ \\
		critic learning rate & $5 \cdot 10^{-3}$ with ADAM optimizer \\        
		max replay size & $5 \cdot 10^5$ \\
		initial replay size & $128$ \\
		batch size & $64$ \\
		soft update & $\tau = 5 \cdot 10^{-3}$ \\
		policy updates & $2.5 \cdot 10^5$ \\
		\hline        
		& \\ & \\        
        
        \textbf{DDPG / TD3} & \\
        \hline
        discount factor $\gamma$ & $0.99$ \\
        rollout steps & $500$ \\
        actor  & neural network parameterized by $\bm{\theta}_{\textrm{actor}}$\\
               & $1$ hidden layer, $50$ units, ReLU activations \\
        actor output & $2 \tanh(f_{\bm{\theta}_{\textrm{actor}}}(\state))$ \\
        actor learning rate & $10^{-3}$ with ADAM optimizer \\
        critic  & neural network parameterized by $\bm{\theta}_{\textrm{critic}}$\\
                & $2$ hidden layers, $50$ units, ReLU activations \\
        critic output & $f_{\bm{\theta}_{\textrm{critic}}}(\state, \action)$ \\
        critic learning rate & $10^{-2}$ with ADAM optimizer \\        
        max replay size & $5 \cdot 10^5$ \\
        initial replay size & $128$ \\
        batch size & $64$ \\
        soft update & $\tau = 5 \cdot 10^{-3}$ \\
        policy updates & $2.5 \cdot 10^5$ \\
        \hline        
        & \\ & \\
%        
%        
%        \textbf{DDPG Offline} & \\
%        \hline
%        dataset sizes & $10^2$, $5 \cdot 10^2$, $10^3$, $2 \cdot 10^3$, $5 \cdot 10^3$, $7.5 \cdot 10^3$, \\
%                      &  $10^4$, $1.2 \cdot 10^4$, $1.5 \cdot 10^4$, $2 \cdot 10^4$, $2.5 \cdot 10^4$ \\
%        discount factor $\gamma$ & $0.97$ \\
%        actor  & neural network parameterized by $\bm{\theta}_{\textrm{actor}}$\\
%               & $1$ hidden layer, $50$ units, ReLU activations \\
%        actor output & $2 \tanh(f_{\bm{\theta}_{\textrm{actor}}}(\state))$ \\
%        actor learning rate & $10^{-2}$ with ADAM optimizer \\
%        critic  & neural network parameterized by $\bm{\theta}_{\textrm{critic}}$\\
%                & $1$ hidden layer, $50$ units, ReLU activations \\
%        critic output & $f_{\bm{\theta}_{\textrm{critic}}}(\state, \action)$ \\
%        critic learning rate & $10^{-2}$ with ADAM optimizer \\
%        soft update & $\tau = 10^{-3}$ \\
%        policy updates & $2 \cdot 10^3$ \\
%        \hline
%        & \\ & \\

        \textbf{PWIS} & \\
        \hline
        dataset sizes & $10^2$, $5 \cdot 10^2$, $10^3$, $2 \cdot 10^3$, $5 \cdot 10^3$, $7.5 \cdot 10^3$, \\
                      &  $10^4$, $1.2 \cdot 10^4$, $1.5 \cdot 10^4$, $2 \cdot 10^4$, $2.5 \cdot 10^4$ \\        
        discount factor $\gamma$ & $0.99$ \\
        policy & neural network parameterized by $\bm{\theta}$\\
               & $1$ hidden layer, $50$ units, ReLU activations \\
        policy output & $\mu = 2 \tanh(f_{\bm{\theta}}(\state))$, $\sigma = \textrm{sigmoid}(g_{\bm{\theta}}(\state))$ \\               
        learning rate  & $10^{-2}$ with ADAM optimizer \\
        policy updates & $2 \cdot 10^3$ \\
        \hline
        & \\ & \\ & \\
        
        \textbf{BEAR} & \\
        \hline
        dataset sizes & $10^2$, $2 \cdot 10^2$ $5 \cdot 10^2$, $10^3$, $2 \cdot 10^3$, $5 \cdot 10^3$, \\
        & $10^4$, $2 \cdot 10^4$, $5 \cdot 10^4$, $10^5$ \\          
        discount factor $\gamma$ & $0.99$ \\
        policy & neural network parameterized by $\bm{\theta}$\\
        & $1$ hidden layer, $50$ units, ReLU activations \\
        policy output & $\mu = 2 \tanh(f_{\bm{\theta}}(\state))$, $\sigma = \textrm{sigmoid}(g_{\bm{\theta}}(\state))$ \\               
        learning rate  & $10^{-4}$ \\
        policy updates & $1 \cdot 10^3$ \\
        \hline
        & \\ & \\ & \\
        
        \textbf{BRAC-(dual)} & \\
        \hline
        dataset sizes & $10^2$, $2 \cdot 10^2$ $5 \cdot 10^2$, $10^3$, $2 \cdot 10^3$, $5 \cdot 10^3$, \\
        & $10^4$, $2 \cdot 10^4$, $5 \cdot 10^4$, $10^5$ \\          
        discount factor $\gamma$ & $0.99$ \\
        policy & neural network parameterized by $\bm{\theta}$\\
        & $1$ hidden layer, $50$ units, ReLU activations \\
        policy output & $\mu = 2 \tanh(f_{\bm{\theta}}(\state))$, $\sigma = \textrm{sigmoid}(g_{\bm{\theta}}(\state))$ \\               
        learning rate  & $10^{-3}$ with Adam \\
        policy updates & $5 \cdot 10^4$ \\
        batch size & $\leq 256$ \\
        soft update & $\tau = 5 \cdot 10^{-3}$ \\
        \hline
        & \\ & \\ & \\
        
        \textbf{MOPO} & \\
        \hline
        dataset sizes & $10^2$, $2 \cdot 10^2$ $5 \cdot 10^2$, $10^3$, $2 \cdot 10^3$, $5 \cdot 10^3$, \\
        & $10^4$, $2 \cdot 10^4$, $5 \cdot 10^4$, $10^5$ \\          
        discount factor $\gamma$ & $0.99$ \\
        policy & neural network parameterized by $\bm{\theta}$\\
        & $1$ hidden layer, $50$ units, ReLU activations \\
        policy output & $\mu = 2 \tanh(f_{\bm{\theta}}(\state))$, $\sigma = \textrm{sigmoid}(g_{\bm{\theta}}(\state))$ \\               
        learning rate  & $3 \cdot 10^{-4}$ with Adam \\
        number of epochs & $5 \cdot 10^2$ \\
        batch size & $256$ \\
        soft update & $\tau = 5 \cdot 10^{-3}$ \\
        BNN hidden dims & $64$ \\
        BNN max epochs & $100$ \\
        BNN ensemble size & $7$ \\
        \hline
        & \\ & \\ & \\

		\textbf{MOReL} & \\
		\hline
		dataset sizes & $10^2$, $2 \cdot 10^2$ $5 \cdot 10^2$, $10^3$, $2 \cdot 10^3$, $5 \cdot 10^3$, \\
		& $10^4$, $2 \cdot 10^4$, $5 \cdot 10^4$, $10^5$ \\          
		discount factor $\gamma$ & $0.99$ \\
		policy & neural network parameterized by $\bm{\theta}$\\
		& $1$ hidden layer, $50$ units, ReLU activations \\
		policy output & $\mu = 2 \tanh(f_{\bm{\theta}}(\state))$, $\sigma = \textrm{sigmoid}(g_{\bm{\theta}}(\state))$ \\               
		step size & $0.02$ \\
		number of iterations & $1 \cdot 10^3$ \\
		dynamics hidden dims & $(128, 128)$, ReLU activations \\
		dynamics lr & $0.001$ \\
		dynamics batch-size & $256$ \\	
		dynamics fit-epochs & $25$ \\	
		dynamics num-models & $4$ \\
		\hline        

        \caption[Algorithms configurations for the Pendulum random data experiment]{\textbf{Algorithms configurations for the Pendulum random data experiment}}
        \label{tab:pendulum_random_configs}
            
    \end{longtable}
\end{center}




==> TPAMI-2021 arxiv/experiments/Pendulum_uniform.tex <==
\begin{figure}[t]
\begin{centering}
    \centering
    \includegraphics[scale=0.7]{figures/experiments/pendulum_uniform_samplesize.pdf}
    \caption[Returns in the Pendulum environment with uniform sampling]{\textbf{Returns in the Pendulum environment with uniform sampling} This box plot shows the return obtained by NOPG-D and NOPG-S as a function of the dataset size with samples from an uniform grid. The error bars show the results of 10 trials. The datasets' details are found in \tabref{tab:pendulum_uniform}.}
    \label{fig:pendulum_uniform}
\end{centering}
\end{figure}





==> TPAMI-2021 arxiv/experiments/Pendulum_uniform_configs.tex <==
\textbf{Algorithm details:}
The configuration used for NOPG-D and NOPG-S are listed in Table~\ref{tab:pendulum_uniform_configs}.
\begin{table}[H]
\begin{center}
	\normalsize
    \begin{tabular}{l l}
        \textbf{NOPG} & \\
        \hline
        discount factor $\gamma$ & 0.99 \\
        state $\vec{h}_{\textrm{factor}}$ & $1.0$ $1.0$  $1.0$   \\
        action $ \vec{h}_{\textrm{factor}}$ & $50.0$ \\
        policy & neural network parameterized by $\bm{\theta}$\\
               & 1 hidden layer, 50 units, ReLU activations \\
        policy output & $2 \tanh(f_{\bm{\theta}}(\state))$ (NOGP-D) \\
                      & $\mu = 2 \tanh(f_{\bm{\theta}}(\state))$, $\sigma = \textrm{sigmoid}(g_{\bm{\theta}}(\state))$ (NOGP-S) \\               
        learning rate  & $10^{-2}$ with ADAM optimizer \\
        $N_{\pi}^{\textrm{MC}}$ (NOPG-S) & 15 \\
        $N_{\phi}^{\textrm{MC}}$ & 1 \\
        $N_{\mu_0}^{\textrm{MC}}$ & (non applicable) fixed initial state \\           
        policy updates & $1.5 \cdot 10^3$ \\
        \hline
    \end{tabular}
    \end{center}

    \caption[NOPG configurations for the Pendulum uniform grid experiment]{\textbf{NOPG configurations for the Pendulum uniform grid experiment}
%    This table contains the configurations of NOPG-D and NOPG-S needed to replicate the results from the Pendulum uniform grid experiment (\ref{tab:pendulum_uniform_results}).
    }
    \label{tab:pendulum_uniform_configs}
\end{table}

==> TPAMI-2021 arxiv/experiments/Pendulum_uniform_dataset_configs.tex <==
Tables~\ref{tab:pendulum_uniform} and~\ref{tab:pendulum_uniform_configs} describe the hyper-parameters used to run the experiment shown in the first plot of Figure~\ref{figure:comparison}.

\textbf{Dataset Generation:}
The datasets have been generated using a grid over the state-action spaces $\theta, \dot{\theta}, u$, where $\theta$ and $\dot{\theta}$ are respectively angle and angular velocity of the pendulum, and $u$ is the torque applied. 
In Table~\ref{tab:pendulum_uniform} are enumerated the different datasets used.

\begin{table}[H]
\begin{center}
	\normalsize
    \begin{tabular}{c c c c}
        $\#\theta$ & $\#\dot{\theta}$ & $\#u$ & Sample size \\ \hline
        $10$ & $10$ & $2$ & $200$ \\
        $15$ & $15$ & $2$ & $450$ \\
        $20$ & $20$ & $2$ & $800$ \\
        $25$ & $25$ & $2$ & $1250$ \\
        $30$ & $30$ & $2$ & $1800$ \\
        $40$ & $40$ & $2$ & $3200$ \\
        \hline
    \end{tabular}
    \end{center}

    \caption[Pendulum uniform grid dataset configurations]{\textbf{Pendulum uniform grid dataset configurations} This table shows the level of discretization for each dimension of the state space ($\#\theta$ and $\#\dot{\theta}$) and the action space ($\#u$). Each line corresponds to a uniformly sampled dataset, where $\theta \in [-\pi, \pi]$, $\dot{\theta} \in [-8, 8]$ and $u \in [-2, 2]$. The entries under the states' dimensions and action dimension correspond to how many linearly spaced states or actions are to be queried from the corresponding intervals. The Cartesian product of states and actions dimensions is taken in order to generate the state-action pairs to query the environment transitions. The rightmost column indicates the total number of corresponding samples.}
    \label{tab:pendulum_uniform}
\end{table}

==> TPAMI-2021 arxiv/experiments/Pendulum_uniform_table.tex <==
\begin{table}[ht]
\begin{center}
    \begin{tabular}{r r r}
        Sample size & NOPG-D & NOPG-S \\ \hline
        200  & $-3794.9 \pm 11.9$ & $-3788.5 \pm 00.9$  \\
        450  & $-576.3  \pm 03.1$  & $-594.1  \pm 39.8$ \\
        800  & $-572.3  \pm 02.3$  & $-572.8  \pm 03.9$ \\
        1250 & $-567.9  \pm 03.2$  & $-564.2  \pm 01.6$ \\
        1800 & $-472.0  \pm 28.8$  & $-457.9  \pm 26.0$ \\
        3200 & $-415.4  \pm 00.7$  & $-428.0  \pm 26.9$ \\
        \hline
    \end{tabular}
\end{center}

    \caption[Returns in the Pendulum environment with uniform sampling]{\textbf{Returns in the Pendulum environment with uniform sampling} This table presents the returns obtained by NOPG-D and NOPG-S as a function of the dataset size with samples from an uniform grid. Depicted are the mean and 95\% confidence intervals of 10 trials. The datasets' details are found in \tabref{tab:pendulum_uniform}.}
    \label{tab:pendulum_uniform_results}
\end{table}


==> TPAMI-2021 arxiv/experiments/hopper.tex <==
\begin{center}
    \begin{longtable}{l l}
        \textbf{NOPG} & \\
        \hline
        dataset & hopper-expert-v2 \\
        dataset sizes & $3 \cdot 10^3$, $5 \cdot 10^3$, $1 \cdot 10^4$ \\        
        discount factor $\gamma$ & $0.99$ \\
        state $\vec{h}_{\textrm{factor}}$ & $4.0$  \\
        action $ \vec{h}_{\textrm{factor}}$ & $10.0$ \\
        policy & neural network parameterized by $\bm{\theta}$\\
               & $2$ hidden layers, $256$ and $256$ units, ReLU activations \\
        policy output & $\tanh(f_{\bm{\theta}}(\state))$ (NOGP-D) \\
                      & $\mu = \tanh(f_{\bm{\theta}}(\state))$, $\sigma = \textrm{sigmoid}(g_{\bm{\theta}}(\state))$ (NOGP-S) \\               
        learning rate  & $ 3 \cdot 10^{-4}$ with ADAM optimizer \\
        $N_{\pi}^{\textrm{MC}}$ (NOPG-S) & $1$ \\
        $N_{\phi}^{\textrm{MC}}$ & $1$ \\
        $N_{\mu_0}^{\textrm{MC}}$ & $500$ \\
        policy updates & $5 \cdot 10^3$ \\
        \hline
        & \\ & \\
    \end{longtable}
\end{center}

==> TPAMI-2021 arxiv/experiments/maze_d4rl.tex <==
\begin{center}
    \begin{longtable}{l l}
        \textbf{NOPG} & \\
        \hline
        dataset sizes & $10^2$, $3.5 \cdot 10^2$, $5 \cdot 10^2$, $6.5 \cdot 10^2$, $8 \cdot 10^2$, $1 \cdot 10^3$ \\        
        discount factor $\gamma$ & $0.99$ \\
        state $\vec{h}_{\textrm{factor}}$ & $2.0$  \\
        action $ \vec{h}_{\textrm{factor}}$ & $5.0$ \\
        policy & neural network parameterized by $\bm{\theta}$\\
               & $2$ hidden layers, $64$ and $32$ units, ReLU activations \\
        policy output & $5 \tanh(f_{\bm{\theta}}(\state))$ (NOGP-D) \\
                      & $\mu = 5 \tanh(f_{\bm{\theta}}(\state))$, $\sigma = \textrm{sigmoid}(g_{\bm{\theta}}(\state))$ (NOGP-S) \\               
        learning rate  & $ 3\cdot 10^{-4}$ with ADAM optimizer \\
        $N_{\pi}^{\textrm{MC}}$ (NOPG-S) & $1$ \\
        $N_{\phi}^{\textrm{MC}}$ & $1$ \\
        $N_{\mu_0}^{\textrm{MC}}$ & $50$ \\
        policy updates & $5 \cdot 10^3$ \\
        \hline
        & \\ & \\
        
        \textbf{BEAR} & \\
        \hline
        dataset sizes & $10^2$, $2 \cdot 10^2$ $5 \cdot 10^2$, $10^3$, $2 \cdot 10^3$, $5 \cdot 10^3$, \\
        & $10^4$, $2 \cdot 10^4$, $5 \cdot 10^4$, $10^5$ \\          
        discount factor $\gamma$ & $0.99$ \\
        policy & neural network parameterized by $\bm{\theta}$\\
        & $2$ hidden layer, $64$ and $32$ units, ReLU activations \\
        policy output & $\mu = 5 \tanh(f_{\bm{\theta}}(\state))$, $\sigma = \textrm{sigmoid}(g_{\bm{\theta}}(\state))$ \\               
        learning rate  & $10^{-4}$ \\
        policy updates & $10^3$ \\
        \hline
        & \\ & \\ 
        
        \textbf{BRAC-(dual)} & \\
        \hline
        dataset sizes & $10^2$, $2 \cdot 10^2$ $5 \cdot 10^2$, $10^3$, $2 \cdot 10^3$, $5 \cdot 10^3$, \\
        & $10^4$, $2 \cdot 10^4$, $5 \cdot 10^4$, $10^5$ \\          
        discount factor $\gamma$ & $0.99$ \\
        policy & neural network parameterized by $\bm{\theta}$\\
        & $2$ hidden layer, $64$ and $32$ units, ReLU activations \\
        policy output & $\mu = 5 \tanh(f_{\bm{\theta}}(\state))$, $\sigma = \textrm{sigmoid}(g_{\bm{\theta}}(\state))$ \\               
        learning rate  & $10^{-3}$ with Adam \\
        policy updates & $5 \cdot 10^4$ \\
        batch size & $\leq 256$ \\
        soft update & $\tau = 5 \cdot 10^{-3}$ \\
        \hline
        & \\ & \\ 
                
        \textbf{MOPO} & \\
        \hline
        dataset sizes & $10^2$, $2 \cdot 10^2$ $5 \cdot 10^2$, $10^3$, $2 \cdot 10^3$, $5 \cdot 10^3$, \\
        & $10^4$, $2 \cdot 10^4$, $5 \cdot 10^4$, $10^5$ \\          
        discount factor $\gamma$ & $0.99$ \\
        policy & neural network parameterized by $\bm{\theta}$\\
        & $2$ hidden layer, $64$ and $32$ units, ReLU activations \\
        policy output & $\mu = 5 \tanh(f_{\bm{\theta}}(\state))$, $\sigma = \textrm{sigmoid}(g_{\bm{\theta}}(\state))$ \\               
        learning rate  & $3 \cdot 10^{-4}$ with Adam \\
        number of epochs & $5 \cdot 10^2$ \\
        batch size & $256$ \\
        soft update & $\tau = 5 \cdot 10^{-3}$ \\
        BNN hidden dims & $64$ \\
        BNN max epochs & $100$ \\ 
        BNN ensemble size & $7$ \\
        \hline
		& \\ & \\ & \\

		\textbf{MOReL} & \\
		\hline
		dataset sizes & $10^2$, $2 \cdot 10^2$ $5 \cdot 10^2$, $10^3$, $2 \cdot 10^3$, $5 \cdot 10^3$, \\
		& $10^4$, $2 \cdot 10^4$, $5 \cdot 10^4$, $10^5$ \\          
		discount factor $\gamma$ & $0.99$ \\
		policy & neural network parameterized by $\bm{\theta}$\\
		& $(64, 32)$, ReLU activations \\
		policy output & $\mu = 5 \tanh(f_{\bm{\theta}}(\state))$, $\sigma = \textrm{sigmoid}(g_{\bm{\theta}}(\state))$ \\               
		step size & $0.005$ \\
		number of iterations & $500$ \\
		dynamics hidden dims & $(32, 32)$, ReLU activations \\
		dynamics lr & $0.001$ \\
		dynamics batch-size & $256$ \\	
		dynamics fit-epochs & $25$ \\	
		dynamics num-models & $4$ \\
		\hline        
        
        

        \caption[Algorithms configurations for the CartPole random data experiment]{\textbf{Algorithms configurations for the CartPole random data experiment}.}
        \label{tab:cartpole_random_configs}
            
    \end{longtable}
\end{center}

==> TPAMI-2021 arxiv/sections/abstract.tex <==
% 1> What is our problem?
Off-policy Reinforcement Learning (RL) holds the promise of better data efficiency as it allows sample reuse and potentially enables safe interaction with the environment.
Current off-policy policy gradient methods either suffer from high bias or high variance, delivering often unreliable estimates.
% 2> Why is this important?
The price of inefficiency becomes evident in real-world scenarios such as interaction-driven robot learning, where the success of RL has been rather limited, and a very high sample cost hinders straightforward application.
% 3> Our suggestion to solve this!
In this paper, we propose a nonparametric Bellman equation, which can be solved in closed form. The solution is differentiable w.r.t the policy parameters and gives access to an estimation of the policy gradient.
% 4> Why does our contribution help
In this way, we avoid the high variance of importance sampling approaches, and the high bias of semi-gradient methods. 
We empirically analyze the quality of our gradient estimate against state-of-the-art methods, and show that it outperforms the baselines in terms of sample efficiency on classical control tasks.


==> TPAMI-2021 arxiv/sections/conclusion.tex <==
In this paper, we presented and analyzed an off-policy gradient technique  \textsl{Nonparametric Off-policy Policy Gradient} (NOPG) \cite{tosatto_nonparametric_2020}. Our estimator overcomes the main issues of the techniques of off-policy gradient estimation. On the one hand, in contrast to semi-gradient approaches, it delivers a full-gradient estimate; and on the other hand, it avoids the high variance of importance sampling by phrasing the problem with nonparametric techniques.
The empirical analysis clearly showed a better gradient estimate in terms of bias, variance, and direction. Our experiments also showed that our method has high sample efficiency and that our algorithm can be behavioral-agnostic and cope with unstructured data.

However, our algorithm, which is built on nonparametric techniques, suffers from the curse of dimensionality. The future work aims to mitigate this problem. We plan to investigate better sparsification techniques united with an adaptive bandwidth. The promising properties of the proposed gradient estimation can, in the future, be adapted to the parametric inference, to extend our approach to the more versatile deep-learning setting.
 

==> TPAMI-2021 arxiv/sections/empirical.tex <==
\label{section:experiments}
In this section, we analyze our method. Therefore, we divide our experiments in two: the analysis of the gradient, and the analysis of the policy optimization using a gradient ascent technique.
The analysis of the gradient comprises an empirical evaluation of the bias, the variance and the gradient direction w.r.t. the ground truth, in relation to some quantities such as the size of the dataset or its degree of ``off-policiness''. 
In the policy optimization analysis, instead, we aim to both compare the sample efficiency of our method in comparison to state-of-the-art policy gradient algorithms, and to study its applicability to unstructured and human-demonstrated datasets.
\subsection{Benchmarking Tasks}
In the following, we give a brief description of the tasks involved in the empirical analysis.
\subsubsection{Linear Quadratic Gaussian Controller}\label{sec:LQG}
A very classical control problem consists of linear dynamics, quadratic reward and Gaussian noise. The main advantage of this control problem relies in the fact that it is fully solvable in closed-form, using the Riccati equations, which makes it appropriate for verifying the correctness of our algorithm.
In our specific scenario, we have a policy encoded with two parameters for illustration purposes. The LQG is defined as
\begin{align}
	\max_{\bm{\theta}} &  \sum_{t=0}^\infty \gamma^t r_t \nonumber \\
	\text{s.t.}\quad  &\state_{t+1} =  A \state_t + B \action_t ;\quad  r_t  = - \state_t^\intercal Q \state_t - \action_t^\intercal R \action_t \nonumber \\
	& \action_{t+1} = \Theta \state_t + \Sigma \epsilon_t; \quad \epsilon_t \sim \mathcal{N}(0, I), \nonumber  
\end{align}  
with $A$, $B$, $Q$, $R$, $\Sigma$ diagonal matrix and $\Theta = \mathrm{diag}(\bm{\theta})$ where $\bm{\theta}$ are considered the policy's parameters.  
%\begin{eqnarray}
%A & = &\begin{bmatrix}
%a_1 & 0 \\
%0 & a_2
%\end{bmatrix}; \quad B = \begin{bmatrix}
%b_1 & 0 \\
%0 & b_2
%\end{bmatrix}; \quad Q =  \begin{bmatrix}
%r_1 & 0 \\
%0 & r_2
%\end{bmatrix}; \nonumber \\
% \quad R  &  = &\begin{bmatrix}
%q_1 & 0 \\
%0 & q_2
%\end{bmatrix}; \quad 
%\Theta  =  \begin{bmatrix}
%\theta_1 & 0 \\
%0 & \theta_2
%\end{bmatrix}; \quad \Sigma  =  \begin{bmatrix}
%\sigma_1 & 0 \\
%0 & \sigma_2
%\end{bmatrix}. \nonumber 
%\end{eqnarray}
In the stochastic policy experiments, $\pi_\theta(\action|\state) = \mathcal{N}(\action | \Theta\state;\Sigma)$, while for the deterministic case $\Sigma=\mathbf{0}$ and $\pi_\theta(\state) = \Theta\state$.
For further details, please refer to the supplementary material.
\subsubsection{OpenAI Pendulum-v0}
The OpenAI Pendulum-v0 \cite{brockman_openai_2016} is a popular benchmark in reinforcement learning. It simulates a simple under-actuated inverted-pendulum. The goal is to swing the pendulum until it reaches the top position, and then to keep it stable.
The state of the system is fully described by the angle of the pendulum $\omega$ and its angular velocity $\dot{\omega}$. The applied torque $\tau \in [-2, 2]$ corresponds to the agent's action.
One of the advantages of such a system, is that its well-known value function is two-dimensional.      
\subsubsection{Quanser Cart-pole}
The cart-pole is another classical task in reinforcement learning. It consists of an actuated cart moving on a track, to which a pole is attached. The goal is to actuate the cart in a way to balance the pole in the top position. 
Differently from the inverted pendulum, the system has a further degree of complexity, and the state space requires the position on the track $x$, the velocity of the cart $\dot{x}$, the angle of the pendulum $\omega$ and its angular velocity $\dot{\omega}$.  
\subsubsection{OpenAI Mountain-Car}
The mountain-car (also known as car-on-hill), consists on an under-powered car that must reach the top of a hill. The car is placed in the valley connecting two hills. In order to reach the goal position, it must first go in opposite direction in order to gain momentum.
Its state is described by the $x$-position of the car, and by its velocity $\dot{x}$. The episodes terminate when the car reaches the goal.
In contrast to the swing-up pendulum, which is hardly controllable by a human-being, this car system is ideal to provide human-demonstrated data.
\reviewAll{
\subsubsection{U-Maze}
U-Maze is an environment from the D4RL dataset \cite{fu_d4rl_2020}. It consist of a simple maze with a 2d shape, where a ball should reach a goal position. The state representation is 4-dimensional (2d position and velocity), and the 2d action represents the velocity of the ball.  
\subsubsection{Hopper}
The Hopper is a popular one-legged robot, with 11-dimensional state and 3-dimensional action space, that should hop forward as fast as possible in a two-dimensional world. We use the implementation offered by MuJoCo \cite{todorov2012mujoco}. Also in this case, we test NOPG on a dataset provided by D4RL.  
}
%\subsubsection{Throttle-Valve System}
%A throttle-valve system is a technical device used for regulating a flow of a fluid or a gas. The control of the throttle-vale is challenging due to its non-linear dynamics.
%Its discretized dynamics are governed by 
%\begin{equation}
%	\mathbf{s}_{t+1} =
%	\state_t + \delta \left(
%	\begin{bmatrix}
%	0 & 1 \\
%	 K_s & K_d  
%	\end{bmatrix}
%	\mathbf{s}_t
%	+
%	\begin{bmatrix}
%	0 \\
%	C_s - K_f \mathrm{sgn}(\omega_t) + \pi_\theta(\mathbf{s_t})
%	\end{bmatrix}\right) \nonumber 
%\end{equation}
%where $\mathbf{s} = [\alpha_t, \omega_t]^\intercal$, $\delta \in \mathbb{R}^+$ represent the discretized time and the policy $\pi_\theta$ is a mapping between a two-dimensional state-space and a one-dimensional action-space.
%This system provides an interesting real-world application of our algorithm, and we will show that our algorithm is able to leverage on the data acquired with an classical optimal-control approach and to obtain better performance.
%\begin{figure}[b]
%	\includegraphics[width=0.975 \columnwidth]{plots/returndet.pdf}
%	\caption{In order to generate off-policy datasets, we interpolate the optimization policy's parameters $(\theta_1, \theta_2)$ with the parameters $(\theta_1', \theta_2')$. On the interpolation lines, the gradient changes both in magnitude and direction. \label{fig:returnlandscape} }
%\end{figure}
\begin{table}[]
	\begin{tabularx}{\linewidth}{|l|L|c|}
		\hline
		\rowcolor{gray!50} Acronym & Description & Typology \\
		\hline
		NOPG-D & Our method with deterministic policy. & \multirow{2}{*}{NOPG}  \\
		\rowcolor{gray!25}\rowcolor{gray!25} NOPG-S &  Our method with stochastic policy. & \cellcolor{white} \\ \hline
		G(PO)MDP+N & G(PO)MDP with normalized importance sampling. & \multirow{2}{*}{PWIS}\\
		\rowcolor{gray!25}G(PO)MDP+BN & G(PO)MDP with normalized importance sampling and generalized baselines. & \cellcolor{white}  \\ \hline
		DPG+Q  & Offline version of the deterministic policy gradient theorem with an oracle for the $Q$-function. & \multirow{2}{*}{SG}    \\
		\rowcolor{gray!25}DDPG & Deep Deterministic Policy Gradient. & \cellcolor{white}\\
		TD3 & Improved version of DDPG. &  \\
		\rowcolor{gray!25}SAC & Soft Actor Critic. &   \cellcolor{white}\\
		BEAR& Bootstrapping Error Accumulation Reduction. &  \\
		\rowcolor{gray!25}BRAC & Behavior Regularized Actor Critic. & \cellcolor{white}  \\
		\hline
		MOPO & Model-based Offline Policy Optimization. &  
		\multirow{2}{*}{MB} \\
		\rowcolor{gray!25}MOReL & Model-Based Offline Reinforcement Learning. &  \cellcolor{white}
		\\
		\hline
	\end{tabularx}
	\caption{Acronyms used in the paper to refer to practical implementation of the algorithms (SG: semi-gradient, PWIS: path-wise importance sampling, MB: model based).\label{table:algorithms}}
\end{table}
\begin{figure}[b]
	\centering
	\includegraphics[width=0.7 \columnwidth]{plots/policies.pdf}
	\caption{Evaluated in the initial state, the optimization policy having parameters $\theta_1, \theta_2$ and the behavioral policy having parameters $\theta_1', \theta_2'$ exhibit a fair distance in probability space.\label{fig:gaussian} }
\end{figure}
 \begin{figure*}[ht!]
 	% \centering
 	\input{plots/pendulum-dataset.tikz}
 	%	\input{plots/gradient-plot.tikz}
 	\input{plots/scatter-gradient.tex}
 	\input{plots/gradient-state-plot.tikz}
 	\caption{\reviewD{(a) The dataset used for the experiment in Section~\ref{sec:trust-region-empirical}. The blue plane represent a policy with constant action. By setting different values of $\theta_3$ we can obtain different policies. For $\theta_3 \approx 0$, the policy is most fitting with the data. (b) When the policy has low log-likelihood, the gradient quickly approaches the zero (i.e., $\|\nabla_\theta \hat{J}_\pi\| \to 0 $). (c) The magnitude of the gradient decreases in low density regions, where the prediction is most uncertain.  }\label{fig:trust-region} }
 \end{figure*}
\subsection{Algorithms Used for Comparisons}
To provide an analysis of the gradient, we compare our algorithm against G(PO)MDP with importance sampling, and with offline DPG (DPG with fixed dataset). Instead of using the na{\"i}ve form of G(PO)MDP with importance sampling, which suffers from high variance, we used the normalized importance sampling \cite{shelton_policy_2013, rubinstein_simulation_2016} (which introduces some bias but drastically reduces the variance), and  the generalized baselines \cite{jie_connection_2010} (which also introduce some bias, as they are estimated from the same dataset). The offline version of DPG, suffers from three different sources of bias: the semi-gradient, the critic approximation and the improper use of the discounted state distribution \cite{thomas_bias_2014,nota_is_2020}. To mitigate these issues and focus more on the semi-gradient contribution to the bias, we provide an oracle $Q$-function (we denote this version as DPG+Q).
\reviewAll{
For the policy improvement, instead, we compare both with online algorithms (Figure~\ref{figure:comparison}) such as TD3 \cite{fujimoto_off-policy_2019} and SAC \cite{haarnoja_soft_2018}, and with offline algorithms (BEAR \cite{kumar_stabilizing_2019}, BRAC \cite{wu_behavior_2019}, MOPO \cite{yu_mopo_2020} and MOReL \cite{kidambi_morel_2020}) as depicted in Figure~\ref{figure:offline-comparison}.}
A full list of the algorithms used in the comparisons with a brief description is available in Table~\ref{table:algorithms}.
%\begin{table}[t]
%	\centering
%	%\rowcolor{2}{gray!25}{white}
%	\begin{tabular}{| l | r r r r r|}\rowcolor{gray!50}
%		\hline
%		Method & 0-40$g$ & 40-80$g$ & 80-120$g$ & 120-150$g$ & Failure \\
%		\hline
%		\rowcolor{white}
%		Demonstrations & 20\% & 33\% & 27\% & 20\% & 0\% \\
%		\rowcolor{gray!25}
%		ProMPs & 43\% & 7\% & 20\% & 17\% & 13\%\\
%		\rowcolor{white}
%		Pro-PriMos & 53\% & 20\% & 3\% & 24\% & 0\\
%		\hline
%	\end{tabular}
%\end{table}
%\subsection{Analysis of the Critic (shall we keep it?)}
%In order to obtain a reliable estimate of the gradient, it is important to obtain a reliable estimation of the critic. In comparison to the vast majority of methods that use either  Monte-Carlo or approximate dynamic programming or a mix of the two, our approach uses a nonparametric closed form solution, using Nadaraya-Watson kernel regression as the approximator. In the literature, there is a little analysis of the performance of such estimator (a more common approach to nonparametric modelling of the Bellman equation has been conduced using Gaussian processes); and therefore we believe in the importance of assessing a bias-variance analysis of our method.
%In order to achieve this objective, we used the LQG system, which allows to retreive the closed-form of the value function, and the OpenAI Sym's Pendulum and Mountain-Car, which are resettable, and their deterministic dynamics allow for a single roll-out estimation.
%Furthermore, using our approach, it is possible to obtain an estimate of the cumulative discounted state-visitation. We will test the accuracy of our state-visit prediction.
 \begin{figure*}[p]
	\centering
	\input{plots/gradient/sample.tikz}\\
	%\vspace{-1em}
	\centering
	\input{plots/gradient/offpolicy.tikz}
	\vspace{-0.5em}
	\caption{Bias, variance, MSE and gradient direction analysis. The MSE plots are equipped with a $95\%$ interval using bootstrapping techniques. The direction analysis plots describe the distribution of angle between the estimates and the ground truth gradient. NOPG exhibits favorable bias, variance and gradient direction compared to PWIS and semi-gradient.\label{fig:sample_analysis}}
\end{figure*}

\subsection{Analysis of the Gradient}
\label{sec:gradient_analysis}
We want to compare the bias and variance of our gradient estimator w.r.t. the already discussed classical estimators.
Therefore, we use the LQG setting described in Section~\ref{sec:LQG}, which allows us to compute the true gradient. Our goal is to estimate the gradient w.r.t. the policy $\pi_\theta$ diagonal parameters $\theta_1, \theta_2$, while sampling from a policy which is a linear combination of $\Theta$ and $\Theta'$. The hyper-parameter $\alpha$ determines the mixing between the two parameters. When $\alpha=1$ the behavioral policy will have  parameters $\Theta'$, while when $\alpha=0$ the dataset will be sampled using $\Theta$.
In Figure~\ref{fig:gaussian}, we can visualize the difference of the
\begin{figure*}[t]
	\centering
	%\hspace{-1.0em}
	\begin{subfigure}[t]{0.5\columnwidth}
		\input{plots/poles/muv0_new.tikz}
	\end{subfigure}
	\hspace{0.8em}
	\begin{subfigure}[t]{0.5\columnwidth}
		\input{plots/poles/v0_new.tikz}
	\end{subfigure}
	\hspace{-1em}
	\begin{subfigure}[t]{0.5\columnwidth}
		\input{plots/poles/muv1_new.tikz}
	\end{subfigure}
	\hspace{-1em}
	\begin{subfigure}[t]{0.5\columnwidth}
		\input{plots/poles/v1_new.tikz}
	\end{subfigure}
	\vspace{-1em}
	\caption{A phase portrait of the state distribution $\tilde{\mu}_{\pi}$ and value function $\tilde{V}_{\pi}$ estimated in the swing-up pendulum task with NOPG-D. Green corresponds to higher values. The two leftmost figures show the estimates before any policy improvement, while the two rightmost show them after $300$ offline updates of NOPG-D. Notice that the algorithm finds a very good approximation of the optimal value function and is able to predict that the system will reach the goal state ($(\omega, \dot{\omega}) = (0, 0) $).}
	\label{figure:muv}
\end{figure*}
 \begin{figure}[t]
	% \centering
	\includegraphics[width=0.9 \columnwidth]{plots/gradient/parametric.pdf}
	\caption{A lower bandwidth corresponds to higher variance, while higher bandwidth increases the bias up to a plateau.\label{fig:parameter} }
\end{figure}
 two policies with parameters $\Theta$ and $\Theta'$. Although not completely disjoint, they are fairly far in the probability space, especially if we take into account that such distance propagates in the length of the trajectories.
\subsubsection{Sample Analysis}
We want to study how the bias, the variance and the direction of the estimated gradient vary w.r.t. the dataset's size. We are particularly interested in the off-policy strategy for sampling, and in this set of experiments we will use constant $\alpha=0.5$. 
Figure~\ref{fig:sample_analysis}a depicts these quantities w.r.t. the number of collected samples. As expected, a general trend for all algorithms is that with a higher number of samples we are able to reduce the variance. The importance sampling based G(PO)MDP algorithms eventually obtain a low bias as well. Remarkably, NOPG has significantly both lower bias and variance, and its gradient direction is also more accurate w.r.t. the G(PO)MDP algorithms (note the different scales of the y-axis). Between DPG+Q and NOPG there is no sensible difference, but we should take into account the already-mentioned advantage of DPG+Q to have access to the true $Q$-function.
%\begin{figure*}
%	\centering
%	\includegraphics[width=1.9\columnwidth]{plots/gradient/stoch-samples.pdf}
%	\caption{Analysis of the gradient w.r.t. the dataset size. In the top row we observe the bias-variance  of the gradient's estimate, corredated with 05\% confidence intervals. On the bottom row, we can observe the distribution of the gradients' directions. It is possible to observe that NOPG exhibits better bias, variance and gradient direction when compared to the importance sampling techniques.}
%\end{figure*}
\subsubsection{Off-Policy Analysis}
We want to estimate the bias and the variance w.r.t. different degrees of ``off-policiness'' $\alpha$, \reviewC{as defined in the beginning of Section~\ref{sec:gradient_analysis}}.
We want to highlight that in the deterministic experiment the behavioral policy remains stochastic. This is needed to ensure the stochastic generation of datasets, which is essential to estimate the bias and the variance of the estimator.
As depicted in Figure~\ref{fig:sample_analysis}, the variance in importance sampling based techniques tends to increase when the dataset is off-policy. On the contrary, NOPG seems to be more subject to an increase of bias. This trend is also noticeable in DPG+Q, where the component of the bias is the one playing a major role in the mean squared error. The gradient direction of NOPG seems however unbiased, while DPG+Q has a slight bias but remarkably less variance (note the different scales of the y-axis). We remark that DPG+Q uses an oracle for the $Q$-function, which supposedly results in lower variance and bias\footnote{Furthermore, we suspect that the particular choice of a LQG task tends to mitigate the problems of DPG, as the fast convergence to a stationary distribution due to the stable attractor, united with the improper discounting, results in a coincidental correction of the state-distribution.}. The positive bias of DPG+Q in the on-policy case ($\alpha=0$) is caused by the improper use of discounting. 
In general, NOPG shows a decrease in bias and variance in order of magnitudes when compared to the other algorithms.
\subsubsection{Bandwidth Analysis}
In the previous analysis, we kept the bandwidth's parameters of our algorithm fixed, even though a dynamic adaptation of this parameter w.r.t. the size of the dataset might have improved the bias/variance trade-off. We are now interested in studying how the bandwidth impacts the gradient estimation. For this purpose, we generated datasets of $1000$ samples with $\alpha=0.5$. We set all the bandwidths of state, action and next state, for each dimension equal to $\kappa$. From Figure~\ref{fig:parameter}, we evince that a lower bandwidth corresponds to a higher variance, while a larger bandwidth approaches a constant bias and the variance tends to zero. This result is in line with the theory.

\reviewB{
\subsubsection{Trust Region}
\label{sec:trust-region-empirical}
In Section~\ref{set:trust-region}, we claimed that the nonparametric technique used has the effect to not consider OOD actions, and more in general, state-action pairs that are in a low density region: in fact the magnitude of the gradient in these regions is low. 
To appreciate this effect, we considered the Pendulum-v0. We generated the data using a Gaussan policy $\mathcal{N}(\bm{\mu}=0, \bm{\Sigma}= 0.2 \mathrm{I})$. Figure~\ref{fig:trust-region}a depicts the generated datataset. Subsequently, we generated a set of linear policies $\avec = \theta_0 \sin \omega + \theta_1 \cos\omega + \theta_2 \dot{\omega} + \theta_3 $ where
the parameters $\theta_0=\theta_1=\theta_2=0$, $\theta_3 \in [-2, 2]$ and $\omega$ and $\dot{\omega}$ represent the angle and the angular velocity of the pendulum. 
When $\theta_3$ is close to $0$, the policy is close to the samples contained in the data, while if $\theta_3$ is close either to $-2$ or $2$, then it is more distant.
In Figure~\ref{fig:trust-region}b shows the estimated policy gradient for different policies. In particular, each point represents the log-likelihood of the policy (w.r.t. the actions contained in the dataset) on the $x$-axis, and the logarithm of the magnitude of the gradient on the $y$-axis. There is a clear correlation between the log-likelihood and the magnitude of the gradient, which tells us that the gradient is close to zero for unlikely policies, supporting, therefore, our claim.
Furthermore, we investigate the contribution of the single state-action pairs to the gradient. The heatmap in Figure~\ref{fig:trust-region}c shows that the highest gradient magnitude appears on the diagonals of the state space. Looking at the generated data, in Figure~\ref{fig:trust-region}a, we notice that the majority of samples are also present on the aforementioned diagonals forming a ``X'' shape. Hence, our experiment shows that the magnitude of the gradient depends also on the density of the state-action space, with lower magnitude in correspondence of lower density of the state space.}
\begin{figure*}[t]
	\begin{subfigure}[t]{0.66\columnwidth}
		\input{plots/poles/pendulumgrid.tikz}
	\end{subfigure}\hspace{0.5em}
	\begin{subfigure}[t]{.66\columnwidth}
		\input{plots/poles/pendulumrand.tikz}
	\end{subfigure}\hspace{-0.5em}
	\begin{subfigure}[t]{.66\columnwidth}
		\input{plots/poles/cartpole.tikz}
	\end{subfigure}
	%	    \begin{subfigure}[t]{.5\columnwidth}
	%			\raisebox{0.87cm}{\includegraphics[height=3.5cm, width=4cm]{plots/poles/real-cart.png}}
	%		\end{subfigure}
	\vspace{-0.2cm}
	\centering
	\input{plots/poles/legend.tikz}
	\caption{Comparison of NOPG in its deterministic and stochastic versions to state-of-the-art \textbf{online} algorithms on continuous control tasks: Swing-Up Pendulum with \textbf{uniform grid} sampling (left), Swing-Up Pendulum  with the \textbf{random agent} (center) and the Cart-Pole stabilization (right). The figures depict the mean and 95\% confidence interval over 10 trials. \myalg~ outperforms the baselines w.r.t the sample complexity. \textbf{Note the log-scale along the $x$-axis}.}
	\label{figure:comparison}
\end{figure*}
\begin{figure*}[t]
	\begin{subfigure}[t]{.66\columnwidth}
		\input{plots/poles/pendulumrand-offline.tikz}
	\end{subfigure}\hspace{-0.5em}
	\begin{subfigure}[t]{.66\columnwidth}
		\input{plots/poles/cartpole-offline.tikz}
	\end{subfigure}
	\begin{subfigure}[t]{0.66\columnwidth}
		\input{plots/poles/maze.tikz}
	\end{subfigure}\hspace{0.5em}
	%	    \begin{subfigure}[t]{.5\columnwidth}
	%			\raisebox{0.87cm}{\includegraphics[height=3.5cm, width=4cm]{plots/poles/real-cart.png}}
	%		\end{subfigure}
	\vspace{-0.2cm}
	\centering
	\input{plots/poles/legend-offline.tikz}
	\caption{Comparison of NOPG in its deterministic and stochastic versions to state-of-the-art \textbf{offline} algorithms on continuous control tasks: Swing-Up Pendulum with \textbf{random agent} (left), the Cart-Pole stabilization (center) and U-Maze with D4RL dataset (right). The figures depict the mean and 95\% confidence interval over 10 trials. \myalg~ is competitive with the sample efficiency of the considered baselines. \textbf{Note the log-scale along the $x$-axis}. }
	\label{figure:offline-comparison}
\end{figure*}
 
\subsection{Policy Improvement}
In the previous section, we analyzed the statistical properties of our estimator. Conversely, in this section, we use the NOPG estimate to fully optimize the policy. 
At the current state, NOPG is a batch algorithm, meaning that it receives as input a set of data, and it outputs an optimized policy, without any interaction with the environment. 
We study the sample efficiency of the overall algorithm. We compare it with both other batch and online algorithms. 
Please notice that online algorithms, such as DDPG-On, TD3 and SAC, can acquire more valuable samples during the optimization process. Therefore, in a direct comparison, batch algorithms are in disadvantage.
\subsubsection{Uniform Grid}
In this experiment we analyze the performance of \myalg~under a uniformly sampled dataset, since, as the theory suggests, this scenario should yield the least biased estimate of NOPG. We generate datasets from a grid over the state-action space of the pendulum environment with different granularities. We test our algorithm by optimizing a policy encoded with a neural-network for a fixed amount of iterations. The policy is composed of a single hidden layer with $50$ neurons and ReLU activations. This configuration is fixed across all the different experiments and algorithms for the remainder of this document.
The resulting policy is evaluated on trajectories of $500$ steps starting from the bottom position.
The leftmost plot in Figure~\ref{figure:comparison}, depicts the performance against different dataset sizes, showing that \myalg~is able to solve the task with $450$ samples. Figure~\ref{figure:muv} is an example of the value function and state distribution estimates of \myalg-D at the beginning and after $300$ optimization steps. The ability to predict the state-distribution is particularly interesting for robotics, as it is possible to predict in advance whether the policy will move towards dangerous states. Note that this experiment is not applicable to PWIS, as it does not admit non-trajectory-based data.
\subsubsection{Comparison with Online Algorithms}
\label{sec:offline-empirical}
In contrast to the uniform grid experiment, here we collect the datasets using trajectories from a random agent in the pendulum and the cart-pole environments. 
In the pendulum task, the trajectories are generated starting from the up-right position and applying a policy composed of a mixture of two Gaussians. The policies are evaluated starting from the bottom position with an episode length of $500$ steps. The datasets used in the cart-pole experiments are collected using a uniform policy starting from the upright position until the end of the episode, which occurs when the absolute value of the  angle $\theta$ surpasses $3\deg$. The optimization policy is evaluated for $10^4$ steps. The reward is $r_t = \cos \theta_t$. Since $\theta$ is defined as $0$ in the top-right position, a return of $10^4$ indicates an optimal policy behavior. 

We analyze the sample efficiency by testing \myalg~in an offline fashion with pre-collected samples, on a different number of trajectories. In addition, we provide the learning curve of DDPG, TD3 and SAC using the implementation in Mushroom \cite{deramo_mushroomrl_2020}. For a fixed size of the dataset, we optimize DDPG-Off and NOPG for a fixed number of steps.  For NOPG, which is offline, we select the policy from the last optimization step.
The two rightmost plots in Figure~\ref{figure:comparison} highlight that our algorithm has superior sample efficiency by more than one order of magnitude w.r.t. the considered online algorithms (note the log-scale on the x-axis).

To validate the resulting policy learned in the simulated cartpole (Figure~\ref{fig:tasks}), we apply the final learned controller on a real Quanser cart-pole, and observe a successful stabilizing behavior as can be seen in the supplementary video.

\reviewAll{
\subsubsection{Comparison with Offline Algorithms}
We use the same environments provided in Section~\ref{sec:offline-empirical} to compare against state-of-the-art offline algorithms. To this end, we used the same datasets on Cart-Pole and Pendulum-v0 to train BRAC, BEAR, MOPO and MOReL. Furthermore, to allow a fairer comparison using the D4RL dataset, we tested our algorithm with the aforementioned baselines on the U-Maze.
To perform the usual sample-analysis, we sub-sampled the dataset in smaller datasets. The results of such analysis can be viewed in Figure~\ref{figure:offline-comparison}. NOPG exhibits a competitive performance w.r.t. the baselines. In more detail, BEAR and MOReL perform suboptimally in our experiments, MOPO perform similarly to NOPG in Pendulum-v0, while failing in Quanser Cart-Pole. BRAC exhibit a similar behavior with our NOPG. All the algorithms seems, however, to fail with the U-Maze, probably due to the scarcity of data, and due to its sparse reward.
} 
\begin{figure}[t]
	\centering
	\begin{subfigure}{0.49\columnwidth}
		\input{plots/Mountain/mountaincar_samplesize_new.tikz}
	\end{subfigure}\hspace{-0.1em}
	\begin{subfigure}{0.49\columnwidth}
		\input{plots/Mountain/mountaincar_trajectories_optimal.tikz}
	\end{subfigure}\vspace{-0.5em}
	%\input{plots/Mountain/legend.tikz}
	\caption{With a small amount of data NOPG is able to reach a policy that surpasses the human demonstrator (dashed line) in the mountain car environment. Depicted are the mean and 95\% confidence over 10 trials (left). An example of a human-demonstrated trajectory and the relative optimized version obtained with \myalg~(right). Although the human trajectories in the dataset are suboptimal, \myalg~converges to an optimal solution (right).}
	\label{figure:mountain}
\end{figure} 
\subsubsection{Human Demonstrated Data}
In robotics, learning from human demonstrations is crucial in order to obtain better sample efficiency and to avoid dangerous policies. This experiment is designed to showcase the ability of our algorithm to deal with such demonstrations without the need for explicit knowledge of the underlying behavioral policy. The experiment is executed in a completely offline fashion after collecting the human dataset, i.e., without any further interaction with the environment. This setting is different from the classical imitation learning and subsequent optimization \cite{kober_policy_2009}.
As an environment we choose the continuous mountain car task from OpenAI. We provide $10$ demonstrations recorded by a human operator and assigned a reward of $-1$ to every step. A demonstration ends when the human operator surpasses the limit of $500$ steps, or arrives at the goal position. The human operator explicitly provides sub-optimal trajectories, as we are interested in analyzing whether \myalg~is able to take advantage of the human demonstrations to learn a better policy than that of the human, without any further interaction with the environment. To obtain a sample analysis, we evaluate NOPG on randomly selected sub-sets of the trajectories from the human demonstrations. Figure~\ref{figure:mountain} shows the average performance as a function of the number of demonstrations as well as an example of a human-demonstrated trajectory. \reviewD{A vanilla behavioral cloning approach trained with the whole dataset leads to a worse performance w.r.t. the human demonstrator. In fact, by simply replicating the demonstrator, the cloned behavior is most of the times not able to reach the flag.}
Notice that both \myalg-S and \myalg-D manage to learn a policy that surpasses the human operator's performance and reach the optimal policy with two demonstrated trajectories. 

\reviewAll{
\subsubsection{Test on a Higher-Dimension Task}
All the considered tasks, are relatively low dimensional, with the higher-dimension of 6, accounting for both states and actions, in the U-Maze.
We tested NOPG also on the Hopper, using the D4RL dataset. NOPG improves w.r.t. the number of samples provided, altough it does not reach a satisfactoy policy (Figure~\ref{figure:hopper}). 
The low performance is probably caused by the poor scaling to high dimensions of nonparametric methods, and the typical need of a large amount of samples due to the complexity of the considered task.}
\begin{figure}[t]
	\begin{subfigure}[t]{0.95\columnwidth}
		\input{plots/poles/hopper.tikz}
	\end{subfigure}
%	\begin{subfigure}[t]{0.45\columnwidth}
%		\input{plots/poles/hopper.tikz}
%	\end{subfigure}
	%	    \begin{subfigure}[t]{.5\columnwidth}
	%			\raisebox{0.87cm}{\includegraphics[height=3.5cm, width=4cm]{plots/poles/real-cart.png}}
	%		\end{subfigure}
	\vspace{-0.2cm}
	\centering
	\input{plots/poles/legend-hopper.tikz}
	\caption{Performance of NOPG on the Hopper-v0, using the D4RL dataset.}
	\label{figure:hopper}
\end{figure}

\reviewB{
\subsection{Computational Complexity}
Our nonparametric approach involves a layer of computation that is not usual in classic deep reinforcement learning solutions. In particular, the construction of the matrix $\approxx{\mathbf{P}}_{\pi}^\gamma$ and the inversion of $\bm{\Lambda}_{\pi}$ can be expensive. 
In the following, we analyze the computational resources required by NOPG.
In particular, we use different sizes of the Pendulum-v0 dataset and investigate the time required to compute an iteration of Algorithm~\ref{alg:kbpgalg}. 
As stated in Section~\ref{sec:gradient-estimation}, the iteration time grows quadratically w.r.t. the number of samples contained in the dataset. The computational cost can be lowered by lowering the number of non-zero element of the matrix $\approxx{\mathbf{P}}_{\pi}^\gamma$ (Figure~\ref{fig:complexity}).
However, while our algorithm considers all the samples at every iteration, classic deep reinforcement learning algorithms usually consider only a fixed amount of data (called "mini batch"), and the computational cost of the iterations results, therefore, to be constant. }

\begin{figure}
	\input{plots/time-complexity.tex}
	\caption{\reviewB{For a fixed amount $k$ of non-zero elements per row of the transition matrix, the iteration time grows quadratically w.r.t. the number of samples. A lower $k$ requires a shorter iteration time.} \label{fig:complexity}}	
\end{figure}



% \subsubsection{An inustrial Application}

==> TPAMI-2021 arxiv/sections/gradient.tex <==
In this section, we introduce a nonparametric Bellman equation with a closed form solution, which carries the dependency from the policy's parameters. We derive the gradient of the solution, and discuss the properties of the proposed estimator.
\subsection{A Nonparametric Bellman Equation}
\reviewC{Nonparametric methods, require the storage of all samples to make predictions, but usually exhibit a low bias. They gained popularity thanks to their general simplicity and their theoretical properties.
In this paper, we focus on kernel density estimation, and Nadaraya-Watson kernel regression. In this context, it is usual to assume the kernel to be a symmetric, real function $\kappa$, with positive co-domain and with $\int k(x, y) \de x = 1$~$\forall y$.
The goal of kernel density estimation is to predict the density of a distribution $p(\state)$. After the collection of $n$ samples $\xvec_i \sim p(\cdot)$, it is possible to obtain the estimated density 
\begin{equation}
	\hat{p}(\xvec) = n^{-1} \sum_{i=1}^n\kappa(\xvec, \xvec_i). \nonumber
\end{equation}
Nadaraya-Watson kernel regression builds on the kernel density estimation to predict the output of a function $f:\mathbb{R}^d\to\mathbb{R}$, assuming to observe a dataset of $n$ samples $\{\xvec_i, y_i\}_{i=1}^n$ with $\xvec_i \sim p(\cdot)$ and $y_i = f(\xvec_i) + \epsilon_i$ (where $\epsilon_i$ is a zero-mean noise with finite variance). The prediction 
\begin{equation}
	\hat{f}(\xvec) = \frac{\int_{\mathbb{R}} y \hat{p}(\xvec, y)\de y}{\hat{p}(\xvec)} = \frac{\sum_{i=1}^n y_i \kappa(\xvec, \xvec_i)}{\sum_{i=1}^n\kappa(\xvec, \xvec_i)} \nonumber
\end{equation}
is constructed on the expectation of the conditional density probability, keeping in account that $\int_{\mathbb{R}} y \kappa(y, y_i) \de y = y_i$.
}
Nonparametric Bellman equations have been developed in a number of prior works. \cite{ormoneit_kernel-based_2002,xu_kernel-based_2007,engel_reinforcement_2005} used nonparametric models such as Gaussian Processes for approximate dynamic programming. \cite{taylor_kernelized_2009} have shown that these methods differ mainly in their use of regularization. \cite{kroemer_non-parametric_2011} provided a Bellman equation using kernel density-estimation and a general overview on nonparametric dynamic programming. In contrast to prior work, our formulation preserves the dependency on the policy, enabling the computation of the policy gradient in closed-form. Moreover, we upper-bound the bias of the Nadaraya-Watson kernel regression to prove that our value function estimate is consistent w.r.t. the classical Bellman equation under smoothness assumptions. \label{nppg}
We focus on the maximization of the average return in the infinite horizon case formulated as a starting state objective  $\int_\state \mu_0(\state)V_\pi(\state) \de \state $ \cite{sutton_policy_2000}.
\begin{definition}
	The discounted infinite-horizon objective is defined by $J_{\pi} = \int \mu_{0}(\state)V_{\pi}(\state)\de \state$. Under a stochastic policy the objective is subject to the Bellman equation constraint
	\label{definition:objective}
	\begin{align}
	V_{\pi}(\state)&\!=\!\int_{\Aset} \pi_{\theta}(\action|\state) \bigg(r(\state,\action)  +\gamma\!\int_{\Sset} V_{\pi}(\nextstate)p(\nextstate|\state, \action)\de \nextstate \bigg)\!\de \action,
	\end{align}
	while in the case of a deterministic policy the constraint is given as
	\begin{equation*}
	V_{\pi}(\state) = r(\state,\pi_{\theta}(\state)) + \gamma \int_{\Sset} V_{\pi}(\nextstate)p(\nextstate|\state, \pi_{\theta}(\state))\de \nextstate.
	\end{equation*}
\end{definition}
Maximizing the objective in Definition~\ref{definition:objective} analytically is not possible, excluding special cases such as under  linear-quadratic assumptions \cite{borrelli_predictive_2017}, or finite state-action space. Extracting an expression for the gradient of $J_{\pi}$ w.r.t. the policy parameters $\theta$ is also not straightforward given the infinite set of possibly non-convex constraints represented in the recursion over $V_{\pi}$. Nevertheless, it is possible to transform the constraints in Definition~\ref{definition:objective} to a finite set of linear constraints via nonparametric modeling, thus leading to an expression of the value function with simple algebraic manipulation \cite{kroemer_non-parametric_2011}.
\subsubsection{Nonparametric Modeling.} 
Assume a set of $n$ observations $D\!\equiv\!\{\state_i, \action_i, r_i, {\nextstate}_i, \gamma_i\}_{i=1}^{n}$ sampled from interaction with an environment, with $\state_i, \action_i \sim \beta(\cdot, \cdot)$, $\state_i' \sim p(\cdot |\state_i, \action_i)$, $r_i \sim R(\state_i, \action_i)$ and $\gamma \sim \gamma(\state_i, \action_i, \nextstate_i)$. We define the kernels $\psi:\Sset\times\Sset \to \mathbb{R}^+$, $\varphi:\Aset\times\Aset\to \mathbb{R}^+$ and $\phi:\Sset\times\Sset\to\mathbb{R}^+$, as normalized, symmetric and positive definite functions with bandwidths $\hvec_{\psi}, \hvec_{\varphi}, \hvec_{\phi}$ respectively. We define $\psi_i(\state) = \psi(\state, \state_i)$, $\varphi_i(\action) = \varphi(\action, \action_i)$, and $\phi_i(\state) = \phi(\state, {\nextstate}_i)$. Following \cite{kroemer_non-parametric_2011}, the mean reward $r(\state, \action)$ and the transition conditional $p(\nextstate|\state, \action)$ are approximated by the Nadaraya-Watson regression \cite{nadaraya_estimating_1964,watson_smooth_1964} and kernel density estimation, respectively
\begin{align}
\approxx{r}(\state, \action) &\! \defeq \! \frac{\sum_{i=1}^n\psi_i(\state)\varphi_i(\action)r_i}{ \sum_{i=1}^n\psi_i(\state)\varphi_i(\action)}\nonumber , \\ 
\approxx{p}(\nextstate | \state, \action) &\! \defeq \! \frac{\sum_{i=1}^n \phi_i(\nextstate)\psi_i(\state)\varphi_i(\action)}{\sum_{i=1}^n \psi_i(\state)\varphi_i(\action)} \nonumber , \\
\approxx{\gamma}(\state, \action, \nextstate) & \defeq
\frac{ \sum_{i=1}^n\gamma_i\psi_i(\state)\varphi_i(\action)\phi_i(\nextstate)}{\sum_{i=1}^n\psi_i(\state)\varphi_i(\action)\phi_i(\nextstate)}\nonumber 
\end{align}
and, therefore, by the product of $\approxx{p}$ and $\approxx{\gamma}$ we obtain
\begin{eqnarray}
	\approxx{p}_{\gamma}(\nextstate |\state, \action) &\defeq& \approxx{p}(\nextstate | \state, \action)\approxx{\gamma}(\state, \action, \nextstate) \nonumber \\
	&=& \frac{ \sum_{i=1}^n\gamma_i\psi_i(\state)\varphi_i(\action)\phi_i(\nextstate)}{\sum_{i=1}^n\psi_i(\state)\varphi_i(\action)}. \nonumber 
\end{eqnarray}

Inserting the reward and transition kernels into the Bellman Equation for the stochastic policy case we obtain the nonparametric Bellman equation (NPBE)
\begin{align}
\approxx{V}_{\pi}(\svec) &\!=\!\int_{\Aset} \! \pis(\avec|\svec)\bigg(\approxx{r}(\state, \action)\!+\!\int_{\Sset} \approxx{V}_{\pi}(\svec')\approxx{p}_\gamma(\svec'|\svec, \avec) \de \svec'\bigg)\!\de \avec \nonumber \\
& \!=\!\sum_i \int_{\Aset}  \frac{\pis(\avec|\svec) \psi_i(\state)\varphi_i(\action)}{\sum_j\psi_j(\state)\varphi_j(\action)}\de \avec \nonumber \\
& \quad \quad \quad \times \bigg(r_i + \gamma_i \int_{\Sset} \phi_i(\svec')\approxx{V}_{\pi}(\svec') \de \svec' \bigg). \label{equation:npbe} 
\end{align}
Equation~\eqref{equation:npbe} can be conveniently expressed in matrix form by introducing the vector of responsibilities $\varepsilon_i(\state)\!=\!\int \pis(\avec|\svec)\! \psi_i(\state)\varphi_i(\action)/\sum_j\psi_j(\state)\varphi_j(\action)\de \avec$, which assigns each state $\state$ a weight relative to its distance to a sample $i$ under the current policy.
\begin{definition}{}
	\label{definition:npbe}
	The nonparametric Bellman equation on the dataset $D$ is formally defined as
	\begin{equation}
	\approxx{V}_{\pi}(\svec)\!=\!\bm{\varepsilon}_{\pi}^{\intercal}(\svec) \left(\rvec +  \int_{\Sset} \phivec_\gamma(\svec')\approxx{V}_{\pi}(\svec') \de \svec' \right), \label{eq:formalnpbe}
	\end{equation}
	with $\phivec_\gamma(\svec)  \!=\![\gamma_1\phi_1(\svec),\dots, \gamma_n\phi_n(\svec)]^{\intercal}, \rvec  \!=\![r_1,\dots, r_n]^{\intercal}$, $\bm{\varepsilon}_{\pi}(\svec)   \!=\![\varepsilon_1^\pi(\svec)$, \dots,  $\varepsilon_n^\pi(\svec)]^{\intercal}$,
	\begin{align}
		\varepsilon_i(\svec, \avec) & = \frac{\psi_i(\state)\varphi_i(\action)}{\sum_j\psi_j(\state)\varphi_j(\action)} \nonumber
	\end{align}
	and
	\begin{align}
		\varepsilon^{\pi}_i(\svec)\!  &= \! \begin{cases}
			\int \pis(\avec|\svec)\varepsilon_i(\svec, \avec)  \de \avec & \text{if $\pi$ is stochastic} \\  \varepsilon_i(\svec, \pis(\svec))  & \text{otherwise.} \nonumber
		\end{cases}
	\end{align}
	% 	\begin{equation}
	% 		\begin{cases}
	% 			\varepsilon^{\pi}_i(\svec) \defeq \int \pis(\avec|\svec) \frac{\psi_i(\state)\varphi_i(\action)}{\sum_j\psi_j(\state)\varphi_j(\action)}\de \avec & \text{if $\pi$ is stochastic}, \\
	% 			\varepsilon^{\pi}_i(\svec)  \defeq \frac{\psi_i(\state)\varphi_i(\pis(\svec))}{\sum_j\psi_j(\state)\varphi_j(\pis(\svec))}                                & \text{otherwise.}
	% 		\end{cases}\nonumber
	% 	\end{equation}
\end{definition}
From Equation~\eqref{eq:formalnpbe} we deduce that the value function must be of the form $\bm{\varepsilon}_{\pi}^\intercal(\state)\qvec$, indicating that it can also be seen as a form of Nadaraya-Watson kernel regression,
\begin{equation}
\bm{\varepsilon}_{\pi}^\intercal(\state)\qvec = \bm{\varepsilon}_{\pi}^{\intercal}(\svec) \left(\rvec +  \int_{\Sset} \phivec_\gamma(\svec')\bm{\varepsilon}_{\pi}^{\intercal}(\svec')\qvec \de \svec' \right). \label{eq:npbewresp}
\end{equation}
Notice that, trivially,  every $\qvec$ which satisfies 
\begin{equation}
\qvec = \rvec + \int_{\Sset} \phivec_\gamma(\svec')\bm{\varepsilon}_{\pi}^{\intercal}(\svec')\qvec \de \svec' \label{eq:npbeworesp}
\end{equation}
also satisfies Equation~\eqref{eq:npbewresp}. Theorem~\ref{theorem:fixedpoint} demonstrates that the algebraic solution of Equation~\eqref{eq:npbeworesp} is the \textsl{only} solution of the nonparametric Bellman Equation~\eqref{eq:formalnpbe}. 
\begin{theorem}{}
	\label{theorem:fixedpoint}
	The nonparametric Bellman equation has a unique fixed-point solution 
	\begin{equation}
	\approxx{V}^*_{\pi}(\svec) \defeq \bm{\varepsilon}^{\intercal}_{\pi}(\svec)\bm{\Lambda}_\pi^{-1}\rvec, \nonumber
	\end{equation} with $\kerres \defeq I-\approxx{\mathbf{P}}_{\pi}^\gamma$ and $\approxx{\mathbf{P}}_\pi^\gamma \defeq \int_{\Sset} \phivec_\gamma(\svec')\bm{\varepsilon}_{\pi}^{\intercal}(\svec') \de \svec' $, where $\bm{\Lambda}_{\pi}$ is always invertible since $\approxx{\mathbf{P}}^{\pi, \gamma}$ is a strictly sub-stochastic matrix (Frobenius' Theorem). The statement is valid also for $n \to \infty$, provided bounded $R$.
\end{theorem}
\reviewD{
The transition matrix $\approxx{\mathbf{P}}_{\pi}^\gamma$ is strictly sub-stochastic since each row $\approxx{\mathbf{P}}_{\pi, i}^\gamma = \gamma_i \int \phi_i(\state')\bm{\varepsilon}_{\pi}^{\intercal}(\svec') \de \svec'$ is composed by the convolution between $\phi_i$, which by definition integrates to one, and $0 \leq \bm{\varepsilon}_{\pi}^{\intercal}(\svec') \leq 1$, as can be seen in Definition~\ref{definition:npbe}.}
Proof of Theorem~\ref{theorem:fixedpoint} is provided in the supplementary material.
\subsection{Nonparametric Gradient Estimation}
\label{sec:gradient-estimation}
With the closed-form solution of $\approxx{V}^*_{\pi}(\svec)$ from Theorem~\ref{theorem:fixedpoint}, it is possible to compute the analytical gradient of \reviewA{$\hat{J}_{\pi}$} w.r.t. the policy parameters
\begin{align}
\grad{\theta} \approxx{V}_{\pi}^*(\svec) &=  \bigg( \pargrad{\theta}\bm{\varepsilon}_{\pi}^{\intercal}(\svec)\bigg)\kerres^{-1} \mathbf{r}  + \bm{\varepsilon}_{\pi}^{\intercal}(\svec) \pargrad{\theta} \kerres^{-1} \mathbf{r}  \nonumber \\
%&= & \bigg( \pargrad{\theta}\bm{\varepsilon}_{\pi}^{\intercal}(\svec)\bigg)\kerres^{-1} \mathbf{r}  - \bm{\varepsilon}_{\pi}^{\intercal}(\svec)\kerres^{-1}\bigg(\pargrad{\theta}\kerres\bigg)\kerres^{-1}\mathbf{r} \nonumber \\
&=  \underbrace{\bigg( \pargrad{\theta}\bm{\varepsilon}_{\pi}^{\intercal}(\svec)\bigg)\kerres^{-1} \mathbf{r}}_{\text{A}} \nonumber \\ &  \quad \quad + \underbrace{  \bm{\varepsilon}_{\pi}^{\intercal}(\svec)\kerres^{-1}\bigg(\pargrad{\theta} \approxx{\mathbf{P}}^\gamma_{\pi}\bigg)\kerres^{-1} \mathbf{r}}_{\text{B}}. \label{equation:kergradv}
\end{align}
Substituting the result of Equation~\eqref{equation:kergradv} into the return specified in Definition~\ref{definition:objective}, introducing $\bm{\varepsilon}_{\pi,0}^{\intercal} \defeq \int\mu_0(\svec)\bm{\varepsilon}_{\pi}^{\intercal}(\svec) \de \svec$, $\mathbf{q}_{\pi} = \bm{\Lambda}^{-1}_\pi \rvec$, and $\bm{\mu}_{\pi} = \bm{\Lambda}_{\pi}^{-\intercal} \bm{\varepsilon}_{\pi,0}$, we obtain
\begin{equation}
\grad{\theta} \approxx{J}_{\pi} = \bigg( \pargrad{\theta}\bm{\varepsilon}_{\pi,0}^{\intercal}\bigg)\mathbf{q}_{\pi}  + \bm{\mu}_{\pi}^{\intercal}\bigg(\pargrad{\theta} \approxx{\mathbf{P}}_{\pi}^\gamma \bigg)\mathbf{q}_{\pi}, \label{equation:algorithmicgradient}
\end{equation}
where $\mathbf{q}_{\pi}$ and $\bm{\mu}_{\pi}$ can be estimated via conjugate gradient to avoid the inversion of $\bm{\Lambda}_\pi$.
It is interesting to notice that \eqref{equation:algorithmicgradient} is closely related to the Policy Gradient Theorem \cite{sutton_policy_2000},
\begin{equation}
\nabla_\theta\hat{J}_\pi =\! \int\displaylimits_{\Sset \times \Aset} \underbrace{\left(\mu_0(\state) +  \bm{\phi}_\gamma^\intercal(\state)\bm{\mu}_\pi\right)}_\text{Stationary distribution}\underbrace{\bm{\varepsilon}^\intercal(\state, \action)\bm{q}_\pi}_{\hat{Q}_\pi(\state, \action)} \nabla_\theta \pi_\theta(\action | \state) \de \action\!\de \state \nonumber
\end{equation} 
and to the Deterministic Policy Gradient Theorem (in its onpolicy formulation) \cite{silver_deterministic_2014},
\begin{equation}
\nabla_\theta \hat{J}_\pi= \int_\Sset \underbrace{\left(\mu_0(\state) + \bm{\phi}_\gamma^\intercal(\state) \bm{\mu}_\pi\right)}_\text{Stationary distribution} \underbrace{\nabla_\action\bm{\varepsilon}^\intercal(\state, \action)\bm{q}_\pi}_{\nabla_\action \hat{Q}_\pi(\state, \action)}  \nabla_\theta \pi_\theta(\state) \de \state . \nonumber 
\end{equation}
In a later analysis, we will consider the state-action surrogate return $J_S^\pi(\state, \action) = (\mu_0(\state) + \Phi_\gamma^\intercal(\state) \bm{\mu}_\pi)\bm{\varepsilon}^\intercal(\state, \action)\bm{q}_\pi$.
The terms $\text{A}$ and $\text{B}$ in Equation~\eqref{equation:kergradv} correspond to the terms in Equation~\eqref{equation:qgrad}. In contrast to semi-gradient actor-critic methods, where the gradient bias is affected by both the critic bias and the semi-gradient approximation \cite{imani_off-policy_2018,fujimoto_off-policy_2019}, our estimate is the \textsl{full gradient} and the only source of bias is introduced by the estimation of $\approxx{V}_{\pi}$, which we analyze in Section~\ref{sec:nonparaestimation}.
The term $\bm{\mu}_\pi$ can be interpreted as the support of the state-distribution as it satisfies  $\bm{\mu}^{\intercal}_\pi =\bm{\varepsilon}_{\pi,0}^{\intercal} + \bm{\mu}_\pi^{\intercal} {\approxx{\mathbf{P}}^\gamma_{\pi}}$. In Section~\ref{section:experiments}, more specifically in Figure~\ref{figure:muv}, we empirically show that $\varepsilon_{\pi}^{\intercal}(\svec)\bm{\mu}_\pi$ provides an estimate of the state distribution over the whole state-space.
%However, we refer to \eqref{equation:algorithmicgradient} for the practical implementation.
The quantities $\bm{\varepsilon}_{\pi,0}^{\intercal}$ and $\approxx{\mathbf{P}}^{\pi}_{i,j}$ are estimated via  Monte-Carlo sampling, which is unbiased but computationally demanding, or using other techniques such as unscented transform or numerical quadrature. The matrix $\approxx{\mathbf{P}}_{\pi}^\gamma$ is of dimension $n \times n$, which can be memory-demanding. In practice, we notice that the matrix is often sparse. By taking advantage of conjugate gradient and sparsification we are able to achieve computational complexity of $\mathcal{O}(n^2)$ per policy update and memory complexity of $\mathcal{O}(n)$. Further details on the computational and memory complexity can be found in the supplementary material. A schematic of our implementation is summarized in Algorithm~\ref{alg:kbpgalg}.
\begin{algorithm}[t]
	\caption{Nonparametric Off-Policy Policy Gradient}
	\label{alg:kbpgalg}
	\begin{algorithmic}
		\STATE \textbf{input:} dataset $\{\state_i, \action_i, r_i,\nextstate_i, \gamma_i \}_{i=1}^{n}$ where $\pi_{\theta}$ indicates the policy to optimize and $\psi, \phi, \varphi$ the kernels respectively for state, action and next-state.
		\WHILE{ \text{not converged}}
		\STATE Compute $\bm{\varepsilon}^{\intercal}_{\pi}(\svec)$ as in Definition~\ref{definition:npbe} and  $\bm{\varepsilon}_{\pi,0}^{\intercal} \defeq \int\mu_0(\svec)\bm{\varepsilon}_{\pi}^{\intercal}(\svec) \de \svec$.
		\STATE Estimate $\approxx{\mathbf{P}}_{\pi}^\gamma$ as defined in Theorem~\ref{theorem:fixedpoint} using MC ($\phi(\svec)$ is a distribution).
		\STATE Solve $\rvec = \bm{\Lambda}_\pi\mathbf{q}_{\pi}$ and $\bm{\varepsilon}_{\pi,0} = \bm{\Lambda}_{\pi}^{\intercal}\bm{\mu}_{\pi}$ for $\mathbf{q}_{\pi}$ and $\bm{\mu}_{\pi}$ using conjugate gradient.
		\STATE Update $\theta$ using Equation~\eqref{equation:algorithmicgradient}.
		\ENDWHILE
	\end{algorithmic}
\end{algorithm}

\subsection{A theoretical Analysis}
\label{sec:nonparaestimation}
Nonparametric estimates of the transition dynamics and reward enjoy favorable properties for an off-policy learning setting. A well-known asymptotic behavior of the Nadaraya-Watson kernel regression,
\begin{align}
& \EV \left[\lim_{n\to \infty}\approxx{f}_n(x) \right] - f(x)  \approx \nonumber\\
& \quad\quad\quad  h^2_n \bigg(\frac{1}{2}f''(x) + \frac{f'(x){ \beta'(x)}}{ \beta(x)}\bigg) \int u^2 K(u)\de u, \nonumber %+o_p(h_n^2) \nonumber
\end{align}
shows how the bias is related to the regression function $f(x)$, as well as to the samples' distribution $\beta(x)$  \cite{fan_design-adaptive_1992,wasserman_all_2006}. 
However, this asymptotic behavior is valid only for infinitesimal bandwidth, infinite samples ($h \to 0, nh \to \infty$) and requires the knowledge of the regression function and of the sampling distribution.

In a recent work, we propose an upper bound of the bias that is also valid for finite bandwidths \cite{tosatto_upper_2020}. 
We show under some Lipschitz conditions that the bound of the Nadaraya-Watson kernel regression bias does not depend on the samples' distribution, which is a desirable property in off-policy scenarios. 
The analysis is extended to multidimensional input space. For clarity of exposition, we report the main result in its simplest formulation, and later use it to infer the bound of the NPBE bias.

\begin{theorem}{}
	\label{theorem:biasnadaraya}
	Let $f\!:\!\mathbb{R}^d\!\to\!\mathbb{R}$ be a Lipschitz continuous function with constant $L_{f}$.
	Assume a set $\{\xvec_i, y_i\}_{i=1}^n$ of i.i.d. samples from a log-Lipschitz distribution $\beta$ with a Lipschitz constant $L_{\beta}$. Assume $y_i = f(\xvec_i) + \epsilon_i$, where $f\!:\!\mathbb{R}^d\!\to\!\mathbb{R}$ and $\epsilon_i$ is i.i.d. and zero-mean. The bias of the Nadaraya-Watson kernel regression with Gaussian kernels in the limit of infinite samples $n\to \infty$ is bounded by
	\begin{equation*}
	\begin{split}
	& \left|\EV \left[\lim_{n\to \infty}\approxx{f}_n(\xvec) \right] - f(\xvec) \right| \leq \\
	& \quad \quad \quad \quad \frac{L_f \sum\limits_{k=1}^d \hvec_k \left(\prod\limits_{i\neq k}^d \chi_i\right)  \left( \frac{1}{\sqrt{2 \pi} } + \frac{L_{\beta}\hvec_k}{2} \chi_k \right) }{ \prod\limits_{i=1}^d \e{\frac{L_{\beta}^2 h_i^2}{2}}\left(1 - \erf\left(\frac{\hvec_i L_{\beta}}{\sqrt{2}} \right) \right)},\\
	\end{split}
	\end{equation*}
	where \begin{equation}
	\chi_i = e^{\frac{L_{\beta}^2\hvec^2_i}{2}}\bigg(1+\erf\bigg(\frac{\hvec_iL_\beta}{\sqrt{2}} \bigg)\bigg) \nonumber ,
	\end{equation}
	$\hvec > 0 \in \mathop{R}^d$ is the vector of bandwidths and $\erf{}$ is the error function.
\end{theorem}

	Building on Theorem~\ref{theorem:biasnadaraya} we show that the solution of the NPBE is consistent with the solution of the true Bellman equation. Moreover, although the bound is not affected directly by $\beta(\state)$, a smoother sample distribution $\beta(\state)$ plays favorably in the bias term (a low $L_{\beta}$ is preferred).
\begin{theorem}{}
	\label{theorem:ultimate}
	Consider an arbitrary MDP $\mathcal{M}$ with a transition density $p$ and a stochastic reward function $R(\svec, \avec) = r(\svec,\avec) + \epsilon_{\svec, \avec}$, where $r(\svec,\avec)$ is a Lipschitz continuous function with $L_R$ constant and $\epsilon_{\svec, \avec}$ denotes zero-mean noise. Assume $|R(\svec, \avec)|\!\leq\!R_{\text{max}}$ and a dataset $D_n$ sampled from a log-Lipschitz distribution $\beta$ defined over the state-action space with Lipschitz constant $L_{\beta}$. Let $V_D$ be the unique solution of a nonparametric Bellman equation with Gaussian kernels $\psi,\varphi,\phi$ with positive bandwidths $\hvec_{\psi},\hvec_{\varphi}, \hvec_{\phi}$ defined over the dataset $\lim_{n\to\infty} D_n$. 
	%$V_D$ is an estimator of the fixed point $V^*$ of the classical Bellman equation defined over $\mathcal{M}$. 
	Assume $V_D$ to be Lipschitz continuous with constant $L_V$. The bias of such estimator is bounded by
	\begin{equation}
	\big|\overline{V}(\svec) - V^*(\svec)\big| \leq  \frac{1}{1-\gamma_c} \bigg(\text{A}_\text{Bias} + \gamma_c L_{V} \sum_{k=1}^{d_s}\frac{h_{\phi,k}}{\sqrt{2 \pi}} \bigg),
	\end{equation}
	where $\overline{V}(\svec) = \EV_{D}[V_D(\svec)]$, $\text{A}_\text{Bias}$ is the bound of the bias provided in Theorem~\ref{theorem:biasnadaraya} with $L_f\!=\!L_R$, $\hvec\!=\![\hvec_{\psi},\hvec_{\varphi}]$, $d\!=\!d_s\!+\!d_a$ and $V^*(\state)$ is the fixed point of the ordinary Bellman equation. \footnote{Complete proofs of the theorems and precise definitions can be found in the supplementary material.}
\end{theorem}
%\vspace{2em}
Theorem~\ref{theorem:ultimate} shows that the value function provided by Theorem~\ref{theorem:fixedpoint} is consistent when the bandwidth approaches infinitesimal values. Moreover, it is interesting to notice that the error can be decomposed in $A_\text{Bias}$, which is the bias component dependent on the reward's approximation, and the remaining term that depends on the smoothness of the value function and the bandwidth of $\phi$, which can be read as the error of the transition's model.

The bound shows that smoother reward functions, state-transitions and sample distributions play favorably against the estimation bias. 
\reviewD{Notice that the bias persist even in the support points. This issue is known in Nadaraya-Watson kernel regression. However, the bias can be controlled and lowered by reducing the bandwidth.
The i.i.d. assumption required by Theorem~\ref{theorem:ultimate} is not restrictive, as even if the samples are collected by a sequential process that interacts with the MPD, the sample distribution will eventually converge to the stationary distribution of the MDP. Furthermore, our algorithm considers all the samples simoultaneously, therefore, some inter-correlations between samples does not affect the estimation.}
\begin{figure}[H]
	\centering
	\includegraphics[width=0.95 \columnwidth]{plots/blocking.pdf}
	\caption{The classic effect (known as boundary-bias) of the Nadaraya-Watson regression predicting a constant function in low-density regions is beneficial in our case, as it prevents the policy from moving in those areas as the gradient gets close to zero. \label{fig:block}}
\end{figure}

\reviewB{
Beyond the bias analysis in the limit of infinite data is important to understand the variance and the bias for finite data.
We provide a finite sample analysis in the empirical section. It is known that the lowest mean squared error is obtained by setting a higher bandwidth in presence of scarce data, and decreasing it with more data. 
In our implementation of NOPG, we select the bandwidth using cross validation.}


\subsubsection{A Trust Region}
\label{set:trust-region}
Very commonly,  in order to prevent harmful policy optimization, the policy is constrained to stay close to the data \cite{peters_relative_2010}, to avoid taking large steps \cite{schulman_trust_2015, schulman_proximal_2017} or to circumvent large variance in the estimation \cite{metelli_policy_2018,chua_deep_2018}. These techniques, which keep the policy updates in a trusted-region, prevent incorrect and dangerous estimates of the gradient.
Even if we do not include any explicit constraint of this kind, the Nadaraya-Watson kernel regression automatically discourages policy improvements towards low-data areas. 
In fact, as depicted in Figure~\ref{fig:block}, the Nadaraya-Watson kernel regression, tends to predict a constant function in low density regions. Usually, this characteristic is regarded as an issue, as it causes the so-called boundary-bias. In our case, this effect turns out to be beneficial, as it constrains the policy to stay close to the samples, where the model is more correct.

%\begin{eqnarray}
%	\| \nabla_\action \varepsilon(\state, \action) \| & = & \left\lVert \nabla_\action \frac{\psi_i(\state)\varphi_i(\action)}{\sum_j\psi_j(\state)\varphi_j(\action)}\right\rVert \nonumber \\
%	& = & \bigg\lVert\frac{\psi_i(\state)\nabla_\action\varphi_i(\action)}{\sum_j\psi_j(\state)\varphi_j(\action)} \nonumber \\
%	&  & - \frac{\psi_i(\state)\varphi_i(\action)}{(\sum_j\psi_j(\state)\varphi_j(\action))^2}\sum_j\psi_j(\state)\nabla_\action\varphi_j(\action) \bigg\rVert \nonumber \\
%	& = &\frac{\psi_i(\state)}{\sum_j\psi_j(\state)\varphi_j(\action)} 
%\end{eqnarray}
%\begin{figure*}[t]
%	\begin{subfigure}[t]{0.5\columnwidth}
%		\input{plots/poles/pendulumgrid.tikz}
%	\end{subfigure}\hspace{0.5em}
%	\begin{subfigure}[t]{.5\columnwidth}
%		\input{plots/poles/pendulumrand.tikz}
%	\end{subfigure}\hspace{-0.5em}
%	\begin{subfigure}[t]{.5\columnwidth}
%		\input{plots/poles/cartpole.tikz}
%	\end{subfigure}
%	\begin{subfigure}[t]{.5\columnwidth}
%		\input{plots/poles/real-cart.tikz}
%	\end{subfigure}
%	%	    \begin{subfigure}[t]{.5\columnwidth}
%	%			\raisebox{0.87cm}{\includegraphics[height=3.5cm, width=4cm]{plots/poles/real-cart.png}}
%	%		\end{subfigure}
%	\vspace{-0.2cm}
%	\centering
%	\vspace{-0.25cm}
%	\input{plots/poles/legend.tikz}
%	\caption{Comparison of NOPG in its deterministic and stochastic versions to state-of-the-art algorithms on continuous control tasks: Swing-Up Pendulum with \textbf{uniform grid} sampling (left), Swing-Up Pendulum  with the \textbf{random agent} (center-left) and the Cart-Pole stabilization (center-right). The figures depict the mean and 95\% confidence interval over 10 trials. \myalg~ outperforms the baselines w.r.t the sample complexity. \textbf{Note the log-scale along the $x$-axis}. The right most picture shows the real cart-pole platform from Quanser.}
%	\label{figure:comparison}
%\end{figure*}

%\begin{figure*}[t]
%	\input{plots/sample-analysis.tex}
%	
%	%	    \begin{subfigure}[t]{.5\columnwidth}
%	%			\raisebox{0.87cm}{\includegraphics[height=3.5cm, width=4cm]{plots/poles/real-cart.png}}
%	%		\end{subfigure}
%	\vspace{-0.2cm}
%	\centering
%	\vspace{-0.25cm}
%	\input{plots/poles/legend.tikz}
%	\caption{Comparison of NOPG in its deterministic and stochastic versions to state-of-the-art algorithms on continuous control tasks: Swing-Up Pendulum with \textbf{uniform grid} sampling (left), Swing-Up Pendulum  with the \textbf{random agent} (center-left) and the Cart-Pole stabilization (center-right). The figures depict the mean and 95\% confidence interval over 10 trials. \myalg~ outperforms the baselines w.r.t the sample complexity. \textbf{Note the log-scale along the $x$-axis}. The right most picture shows the real cart-pole platform from Quanser.}
%	\label{figure:comparison}
%\end{figure*}

==> TPAMI-2021 arxiv/sections/introduction.tex <==
\IEEEPARstart{R}{einforcement learning} has made overwhelming progress in recent years, especially when applied to board and computer games, or simulated tasks \cite{mnih_human-level_2015,haarnoja_soft_2018,schulman_trust_2015}.
 However, in comparison, only a little improvement has been achieved on real-world tasks. 
One of the reasons of this gap is that the vast majority of reinforcement learning approaches are on-policy. On-policy algorithms require that the samples are collected using the optimization policy; and therefore this implies that a) there is little control on the environment and b) samples must be discarded after each policy improvement, causing high sample inefficiency.
In contrast, off-policy techniques are theoretically more sample efficient, because they decouple the procedures of data acquisition and policy update, allowing for the possibility of sample-reuse. Furthermore, off-policy estimation enables offline (or batch) reinforcement learning, which means that the algorithm extracts the optimal policy from a fixed dataset. This property is crucial in many real-world applications, since it allows a decoupled data-acquisition process, and, subsequently, a safer interaction with the environment. However, classical off-policy algorithms like Q-learning with function approximation and its offline version, fitted Q-iteration  \cite{ernst_tree-based_2005,riedmiller_neural_2005}, are not guaranteed to converge \cite{baird_residual_1995,lu_non-delusional_2018}, and allow only discrete actions. More recent semi-gradient\footnote{We adopt the terminology from \cite{imani_off-policy_2018}.} off-policy techniques, like Off-Policy Actor Critic (Off-PAC) \cite{degris_off-policy_2012-1}, Deep Deterministic Policy Gradient (DDPG) \cite{silver_deterministic_2014,lillicrap_continuous_2016}, Soft Actor Critic (SAC) \cite{haarnoja_soft_2018}, often perform sub-optimally, especially when the collected data is strongly off-policy, due to the biased semi-gradient update \cite{fujimoto_off-policy_2019}. 
\reviewAll{In the last years, offline techniques like Conservative Q-Learning (CQL) \cite{kumar_conservative_2020}, Bootstrapping Error Accumulation Reduction (BEAR) \cite{kumar_stabilizing_2019} and  Behavior Regularized Actor Critic (BRAC) \cite{wu_behavior_2019}, take care of a particular treatment of the out-of-distribution (OOD) policy improvement, however, still using the semi-gradient estimation}.
Another class of off-policy gradient estimation uses importance sampling \cite{shelton_policy_2001,meuleau_exploration_2001,peshkin_learning_2002}~to deliver an unbiased estimate of the gradient but suffer from high variance and is generally only applicable with stochastic policies. Moreover, these algorithms require the full knowledge of the behavioral policy, making them unsuitable when data stems from a human demonstrator. 
\begin{figure}[t]
	\centering
	\includegraphics[width=0.95 \columnwidth]{plots/scheme.png}
	\caption{In the off-policy reinforcement learning scheme, the policy can be optimized using an off-policy dataset. This allows for safer interaction with the system and for better sample efficiency.}
	\label{figure:gradient}
\end{figure}
On the other hand, model-based approaches aim to approximate the environment's dynamics, allowing the generation of synthetic samples. The generative model can, in principle, be used by an on-policy reinforcement learning algorithm, therefore, encompassing the difficulty of off-policy estimation.
However, the generation of synthetic samples is also problematic, as they are affected by the error of the approximated dynamics. 
\reviewAll{To mitigate this problem, state-of-the-art techniques aim to quantify and penalize the most uncertain regions of the state-action space, like Model-based Offline Policy Optimization (MOPO) \cite{yu_mopo_2020} and Model-based Offline Reinforcement Learning (MOReL) \cite{kidambi_morel_2020}.} 
\reviewC{To address all previously highlighted issues, we propose a new algorithm, the Nonparametric Off-policy Policy Gradient (NOPG) \cite{tosatto_nonparametric_2020}. NOPG constructs a nonparametric model of the dynamics and the reward signal, and builds a full-gradient estimate based on the closed-form solution of a nonparametric Bellman equation. 
Our approach, in contrast to the majority of model-based approaches, does not require the generation of artificial data.
On the other hand, while model-free approaches are either built on semi-gradient estimation, or importance sampling, NOPG computes a full-gradient estimate without importance sampling estimators, and allows for the use of human demonstrations.} 
%  Unlike other nonparametric methods like PILCO, our approach allows for multimodal state-transitions, and can handle the infinite-horizon setting.
Figure~\ref{figure:gradient} shows the offline scheme of NOPG. A behavioral policy, represented by a human demonstrator, provides (possibly suboptimal) trajectories that solve a task. NOPG optimizes a policy from off-line and off-policy samples. 

\reviewC{\textbf{Contribution.}
This paper introduces a nonparametric Bellman equation, and the full-gradient  derived from its closed-form solution. We study the properties of the nonparametric Bellman equation, focusing on the bias of its closed-form solution.
We empirically analyze the bias and the variance of the proposed gradient estimator. We compare its effectiveness and efficiency w.r.t. state of the art online and offline techniques, observing that NOPG exhibits high sample efficiency.}



 

==> TPAMI-2021 arxiv/sections/problem_statement.tex <==


\section{Problem Statement}
	Consider the reinforcement learning problem of an agent interacting with a given environment, as abstracted by a Markov decision process (MDP) and defined over the tuple $(\Sset, \Aset, \gamma, P, R, \mu_0)$ where $\Sset \equiv \mathbb{R}^{d_s}$ is the state space, $\Aset \equiv \mathbb{R}^{d_a}$ the action space, the transition-based discount factor $\gamma$ is a stochastic mapping between $\Sset\times\Aset\times\Sset$ to $[0, 1)$, which allows for unification of episodic and continuing tasks \cite{white_unifying_2017}. \reviewD{The discount factor allows the transormation of a particular MDP to an equivalent MDP where, at each state-action, there is $1-\gamma$ probability to transition to an absorbing state with zero reward. A variable discount factor, can, therefore, be interpreted as a variable probability of transitioning to an absorbing state. } To keep however the theory simple, we will assume that $\gamma(\state, \action, \state') \leq \gamma_c$ where $\gamma_c < 1$. The transition probability from a state $\state$ to $\nextstate$ given an action $\action$ is governed by the conditional density $\Trans{\nextstate}{\state}{\action}$. The stochastic reward signal $R$ for a transition $(\state, \action, \nextstate) \in \Sset \times \Aset \times \Sset$ is drawn from a distribution $R(\state, \action, \nextstate)$ with mean value $\EV_{\nextstate}[R(\state, \action, \nextstate)] = r(\state, \action)$. The initial distribution $\mu_0(\state)$ denotes the probability of the state $\state \in \Sset$ to be a starting state. 
	A policy $\pi$ is a stochastic or deterministic mapping from $\Sset$ onto $\Aset$, usually  parametrized by a set of parameters $\theta$.
	
	We define an \textsl{episode} as $\tau \equiv \{\state_t, \action_t, r_t, \gamma_t\}_{t=1}^\infty$ where
	\begin{eqnarray}
	& &\mathbf{s}_0 \sim \mu_{0}(\cdot);\quad  \mathbf{a}_t \sim \pi(\cdot \mid \mathbf{s}_t);\quad  \mathbf{s}_{t+1} \sim p(\cdot \mid \mathbf{s}_t, \mathbf{a}_t) \nonumber \\
	& & r_t \sim R(\mathbf{s}_t, \mathbf{a}_t, \state_{t+1});\quad  \gamma_t \sim \gamma(\state_t, \action_t, \state_{t+1}). \nonumber 
	\end{eqnarray}
	In this paper we consider the discounted infinite-horizon setting, where the objective is to maximize the expected return
	\begin{equation}
	J_{\pi}= \EV_\tau\left[\sum_{t=0}^{\infty} r_t \prod_{i=0}^{t}\gamma_i\right] \label{eq:return}.
	\end{equation}
	It is important to introduce two important quantities: the \textsl{stationary state visitation} $\mu_{\pi}$ and the \textsl{value function} $V_{\pi}$.
	We naturally extend the stationary state visitation defined by \cite{sutton_policy_2000} with the transition-based discount factor  
	\begin{eqnarray}
		\mu(\mathbf{s}) = \EV_\tau\left[ \sum_{t=0}^{\infty}  p(\mathbf{s}=\state_t | \pi, \mu_0) \prod_{i=1}^t\gamma_i\right], \nonumber
	\end{eqnarray}
	or, equivalently, as the fixed point of 
	\begin{eqnarray}
		\mu(\mathbf{s}) = \mu_0(\mathbf{s}) +  \int_{\Sset}\int_{\Aset} p_\gamma(\svec | \svec', \avec')\pi(\avec' | \svec')\mu_\pi(\nextstate)\de \svec'\de \avec' \nonumber
	\end{eqnarray}
	where, from now on, $p_\gamma(\nextstate | \state, \action)\! =\! p(\nextstate | \state, \action)\mathbb{E}[\gamma(\state, \action, \nextstate)]$.
	The value function
	\begin{eqnarray}
	V_{\pi}(\svec) = \EV_\tau\left[ \sum_{t=0}^\infty  r_t p(r_t | \svec_0 = \svec,  \pi) \prod_{i=0}^t\gamma_i\right], \nonumber
	\end{eqnarray}
	corresponds to the fixed point of the Bellman equation,
	\begin{equation}
	V_\pi(\svec)  =  \int_{\Aset} \pi(\avec| \svec)\bigg(r(\svec, \avec)+ \int_{\Sset}V_\pi(\svec')p_\gamma(\svec' | \svec, \avec)\de \svec' \bigg)\de \avec . \nonumber
	\end{equation}
	The state-action value function is defined as
	\begin{equation}
		Q_\pi(\svec, \action)  =  r(\svec, \avec) +  \int_{\Sset}V_\pi(\svec')p_\gamma(\svec' | \svec, \avec)\de \svec'. \nonumber
	\end{equation}

	The expected return \eqref{eq:return} can be formulated as
	\begin{eqnarray}
		J_{\pi} = \int_{\Sset} \mu_0(\svec)V_{\pi}(\svec)\de \svec = \int_{\Sset}\int_{\Aset}\mu_\pi(\svec)\pi(\avec | \svec)r(\svec, \avec)\de \avec\de \svec . \nonumber
	\end{eqnarray}

\textbf{Policy Gradient Theorem.} Objective \eqref{eq:return} is usually maximized via gradient ascent. The gradient of $J_{\pi}$ w.r.t. the policy parameters $\theta$ is

\begin{equation*}
\nabla_{\theta}J_{\pi} \!=\! \int\displaylimits_{\Sset}\int\displaylimits_{\Aset}\! \mu_{\pi}(\svec)\pi_{\theta}(\avec|\svec)Q_{\pi}(\svec,\avec)\nabla_{\theta}\log \pi_{\theta}(\avec | \svec) \de \avec \de \svec,
\end{equation*}
as stated in the policy gradient theorem \cite{sutton_policy_2000}. 
When it is possible to interact with the environment with the policy $\pi_\theta$, one can approximate the integral by considering the state-action as a distribution (up to a normalization factor) and use the samples to perform a Monte-Carlo (MC) estimation \cite{williams_simple_1992}. The $Q$-function can be estimated via Monte-Carlo sampling, approximate dynamic programming or by direct Bellman minimization. 
In the off-policy setting, we do not have access to the state-visitation $\mu_\pi$ induced by the policy, but instead we observe a different state distribution.
While estimating the $Q$-function with the new state distribution is well established in the literature \cite{watkins_q-learning_1992, ernst_tree-based_2005}, the shift in the state visitation $\mu_\pi(\state)$ is more difficult to obtain. State-of-the-art techniques either omit to consider this shift (we refer to these algorithms as \textsl{semi-gradient}), or they try to estimate it via importance sampling correction. These approaches will be discussed in detail in Section~\ref{sec:related_work}.



==> TPAMI-2021 arxiv/sections/relatedwork.tex <==
\section{Related Work}
\label{sec:related_work}
\reviewAll{Off-policy and offline policy optimization became increasingly more popular in the recent years and have been explored in many different flavors. Batch reinforcement learning, in the model-free view, has been elaborated both as a value-based and a policy gradient technique (we include actor-critic in this last class). Recently, offline reinforcement learning has been proposed also in the mode-based formulation. In this section, we aim to detail both the advantages and disadvantages of the proposed approaches. As we will see, our solution shares some advantages typical of the model-free policy gradient algorithms while using an approximated model of the dynamics and reward.}
\subsection{Model Free}
\reviewAll{The model-free offline formulation aims to improve the policy based purely on the samples collected in the dataset, without generating synthetic samples from an approximated model. We can divide this broad category in two main families: the value-based approaches, and the policy gradients.}
\subsubsection{Value Based}
\reviewAll{Value-based techniques are constructed on the approximate dynamic theory, leveraging on the policy-improvement theorem and on the contraction property of the Bellman operator. Examples of offline approximate dynamic programming algorithms are Fitted Q-Iteration (FQI) and Neural FQI (NFQI) \cite{ernst_tree-based_2005, riedmiller_neural_2005}. The $\max$ operator used in the optimal Bellman operator, usually restricts the applicability to discrete action spaces (few exceptions, \cite{antos_fitted_2007}). Furthermore, the projected error can prevent the convergence to a satisfying solution \cite{baird_residual_1995}. These algorithms usually suffer also of the delusion bias \cite{lu_non-delusional_2018}.
Despite these issues, there has been a recent revival of value-based techniques in the context of offline reinforcement learning. Batch-Constrained Q-learning (BCQ) \cite{fujimoto_off-policy_2019}, at the best of our knowledge, firstly defined the extrapolation error, which is partially caused by optimizing unseen (out of distribution, OOD) state-action pairs in the dataset. }
This source of bias has been extensively studied in subsequent works, both in the model-free and model-based setting.
\reviewA{ Value-based methods using non-parametric kernel-based approaches have also been used \cite{ormoneit_kernel-based_2002,xu_kernel-based_2007,kroemer_kernel-based_2012}.  An interesting discussion in \cite{taylor_kernelized_2009} shows that kernelized least square temporal difference approaches are also approximating the reward and transition models, and therefore they can be considered model-based.}
\subsubsection{Policy Gradient}
\reviewAll{This class of algorithms leverages their theory on the policy gradient theorem \cite{sutton_policy_2000,silver_deterministic_2014}. Examples of policy gradients are REINFORCE \cite{williams_simple_1992}, G(PO)MDP \cite{baxter_infinite-horizon_2001}, natural policy gradient  \cite{kakade_natural_2001}, and Trust-Region Policy Optimization (TRPO) \cite{schulman_trust_2015}. Often, these approaches make use of approximate dynamic programming to estimate the $Q$-function (or related quantities), to obtain lower variance \cite{peters_natural_2008,lillicrap_continuous_2016,schulman_proximal_2017,haarnoja_soft_2018}. The policy gradient theorem, however, defines the policy gradient w.r.t. \textsl{on-policy samples}. To overcome this problem two main techniques have been introduced: semi-gradient approaches, which rely on the omission of one term in the computation of the gradient, introduce an irreducible source of bias, while importance sampling solutions, which are unbiased, suffer from high variance.}
%Semi-gradient approaches omit one term in the gradient computation, which causes an estimation bias \cite{imani_off-policy_2018}.
%The importance sampling correction, although unbiased, suffers from high variance, which makes it often unpractical \cite{owen_monte_2013}.
%Model based approaches rely on a model's estimation, and optimize the policy following this model. However, the model's error propagates in the number of steps, adding also a significant source of bias \cite{deisenroth_pilco:_2011}.
\begin{figure*}[pht]
	\centering
	\begin{subfigure}[t]{.6\columnwidth}
		\input{plots/poles/lqg.tikz}
	\end{subfigure}
	\hspace{3pt}
	\begin{subfigure}[t]{0.35\columnwidth}
		\input{plots/poles/pendulum.tikz}
	\end{subfigure}
	\hspace{3pt}
	\begin{subfigure}[t]{.5\columnwidth}
		\input{plots/poles/mountain.tikz}
	\end{subfigure}
	\hspace{3pt}
	\begin{subfigure}[t]{.5\columnwidth}
		\input{plots/poles/real-cart.tikz}
	\end{subfigure}
%	\begin{subfigure}[t]{.5\columnwidth}
%		\input{plots/poles/valve.tikz}
%	\end{subfigure}
	\vspace{-0.5cm}
	\caption{Some of the benchmarking tasks. The return's landscape (a) of the LQG problem. In the gradient analysis, we obtain the gradient of the policy with parameters $\theta_1, \theta_2$ by sampling from a policy interpolated with the parameters $\theta_1', \theta_2'$. Sub-figures (b) and (d) depicts the OpenAI environment used. The real system in (c) has been used to evaluate the policy learned to stabilize the cart-pole task.\label{fig:tasks}}
\end{figure*}
\\
\textbf{Semi-Gradient:}
The off-policy policy gradient theorem was the first proposed off-policy actor-critic algorithm \cite{degris_off-policy_2012-1}. Since then, it has been used by the vast majority of state-of-the-art off-policy algorithms \cite{silver_deterministic_2014, lillicrap_continuous_2016, haarnoja_soft_2018}. Nonetheless, it is important to note that this theorem and its successors, introduce two approximations to the original policy gradient theorem \cite{sutton_policy_2000}. First, semi-gradient approaches consider a modified discounted infinite-horizon return objective $\approxx{J}_{\pi} = \int\rho_{\beta}(\svec)V_{\pi}(\svec) \de \state$, where $\rho_{\beta}(\svec)$ is state distribution under the behavioral policy $\pi_{\beta}$. Second, the gradient estimate is modified to be
\begin{align}
\gradt \approxx{J}_{\pi} & = \gradt\int_{\Sset} \rho_{\beta}(\state) V_{\pi}(\state)\de \state \nonumber \\
& = \gradt \int_{\Sset} \rho_{\beta}(\state) \int_{\Aset} \pi_{\theta}(\action|\state) Q_{\pi}(\state, \action)\de \action \de \state  \nonumber                                                 \\
& = \int\displaylimits_{\Sset} \rho_{\beta}(\state) \int\displaylimits_{\Aset} \underbrace{\gradt \pi_{\theta}(\action|\state) Q_{\pi}(\state, \action)}_{\text{A}} \nonumber \\
& \quad \quad + \underbrace{\pi_{\theta}(\action|\state) \gradt Q_{\pi}(\state, \action)}_{\text{B}} \de \action \de \state \label{equation:qgrad} \\
& \approx \int\displaylimits_{\Sset} \rho_{\beta}(\state) \int\displaylimits_{\Aset} \gradt \pi_{\theta}(\action|\state) Q_{\pi}(\state, \action) \de \action\de \state, \nonumber
\end{align}
where the term $\text{B}$ related to the derivative of $Q_{\pi}$ is ignored. The authors provide a proof that this biased gradient, or \textsl{semi-gradient}, still converges to the optimal policy in a tabular setting \cite{degris_off-policy_2012-1, imani_off-policy_2018}. However, further approximation (e.g., given by the critic and by finite sample size), might disallow the convergence to a satisfactory solution.
Although these algorithms work correctly sampling from the replay memory (which discards \textsl{the oldest} samples), they have shown to fail with samples generated via a completely different process \cite{imani_off-policy_2018,fujimoto_off-policy_2019}.
The source of bias introduced in the semi-gradient estimation depends fully on the distribution mismatch, and cannot be recovered by an increment of the dataset size or with a more powerful function approximator. Still, mainly due to its simplicity, semi-gradient estimation has been used in the off-line scenario.
The authors of these works do not tackle the distribution mismatch with its impact to the gradient estimation, but rather consider to prevent the policy taking OOD actions.
In this line of thoughts, Batch-Constrained Q-learning 
(BCQ) \cite{fujimoto_off-policy_2019} introduces a regularization that keeps the policy close to the behavioral policy,
Bootstraping Error Accumulation Reduction (BEAR) \cite{kumar_stabilizing_2019} considers instead a pessimistic estimate of the $Q$ function which penalizes the uncertainty, Behavior Regularized Actor Critic (BRAC) \cite{wu_behavior_2019} proposes instead a generalization of the aforementioned approaches.  
\\
\textbf{Importance-Sampling:}
 One way to obtain an unbiased estimate of the policy gradient in an off-policy scenario is to re-weight every trajectory via importance sampling \cite{meuleau_exploration_2001,shelton_policy_2001, peshkin_learning_2002}. An example of the gradient estimation via G(PO)MDP \cite{baxter_infinite-horizon_2001} with importance sampling is given by
\begin{align}
\nabla_{\theta} J_{\pi} = \mathbb{E}\left[\sum_{t=0}^{T-1} \rho_t \left(\prod_{j=0}^{t-1}\gamma_j\right)r_t \sum_{i=0}^t \nabla_{\theta} \log \pi_{\theta}(\action_i | \state_i) \right] \label{eq:pwis},
\end{align}
where $\rho_t = \prod_{z=0}^{t} \pi_{\theta}(\action_z | \state_z)/\pi_{\beta}(\action_z | \state_z)$.
This technique applies only to stochastic policies and requires the knowledge of the behavioral policy $\pi_\beta$. Moreover, Equation~\eqref{eq:pwis} shows that path-wise importance sampling (PWIS) needs a trajectory-based dataset, since it needs to keep track of the past in the correction term $\rho_t$, hence introducing more restrictions on its applicability.
Additionally, importance sampling suffers from high variance  \cite{owen_monte_2013}. 
Recent works have helped to make PWIS more reliable. For example, \cite{imani_off-policy_2018}, building on the emphatic weighting framework \cite{sutton_emphatic_2016},  proposed a trade-off between PWIS and semi-gradient approaches.  Another possibility consists in restricting the gradient improvement to a safe-region, where the importance sampling does not suffer from too high variance \cite{metelli_policy_2018}. Another interesting line of research is to estimate the importance sampling correction on a state-distribution level instead of on the classic trajectory level \cite{liu_breaking_2018, liu_off-policy_2019, nachum_algaedice:_2019}. We note that despite the nice theoretical properties, all these promising algorithms have been applied on low-dimensional problems, as importance sampling suffers from the curse of dimensionality. 
\\
\subsection{Model-Based}
\reviewAll{
While all model-free offline techniques rely purely on the samples contained in the offline dataset, model-based techniques aim to approximate the transitions from that  dataset. The approximated model is then used to generate new artificial samples.
These approaches do not suffer from the distribution mismatch problem described above, as the samples can be generated on-policy by the model (and therefore, in principle, any online algorithm can  be used). 
This advantage is overshadowed by the disadvantage of having unrealistic trajectories generated by the approximated model.  
For this reason, many recent works focus on discarding unrealistic samples, relying on a pessimistic approach towards uncertainty.
In some sense, we encounter again the problem of quantifying our uncertainty - given the limited information contained in the dataset - and to prevent the policy or the model to use or generate uncertain samples.
In this view, the Probabilistic Ensemble with Trajectory Sampling (PETS) \cite{chua_deep_2018} uses an ensemble of probabilistic models of the dynamics to quantify both the epistemic and the aleatoric uncertainties, and uses model predictive control to act in the real environment.
Model Based Offline Planning (MBOP) \cite{argenson_model-based_2020}  uses a behavioral cloning policy as a prior to the planning algorithm. Plan Online and Learn Offline (POLO) \cite{lowrey2018plan} proposes to learn the value function from a known model of the dynamics and to use model predictive control on the environment. Both Model Based Reinforcement Learning (MOReL) \cite{kidambi_morel_2020} and Model-based Offline Policy Optimization (MOPO) \cite{yu_mopo_2020} learn instead the model to train a parametric policy. MOReL learns a pessimistic version of the real MDP, by partitioning the state-action space in known and unknown and penalizing the policies visiting the unknown region. Instead, MOPO builds a pessimistic MDP by introducing a reward penalization toward model uncertainty.
}

\reviewAll{
NOPG, instead,  provides a theoretical framework built on a nonparametric approximation of the reward and the state transition. Such approximation is used to compute the policy gradient in closed-form. For this reason, our method differs from classic model-based solutions since it does not generate synthetic trajectories.
Most of the state-of-the-art model-free offline algorithms, on the other hand, utilize a biased and inconsistent gradient estimate. Instead, our approach delivers a full-gradient estimate that allows a trade-off between bias and variance. The quality of the gradient estimate results in a particularly sample-efficient policy optimization, as seen in the empirical section.}
%\subsection{Model Based}
%Another natural approach which comes to mind when thinking about off-policy optimization, is to use a learned model of the transition. This model allows to generate new samples and therefore to optimize the policy potentially off-line. The proclaimed efficiency of model-based techniques relies on the fact that they allow off-policy optimization. However, model-based techniques are also problematic: the model error propagates in the Bellman recursion (or in the number of steps, if we prefer), often resulting in bad policy improvements. PILCO \cite{deisenroth_pilco:_2011} aims to optimize the policy using probabilistic inference based on Gaussian Processes to model the estimation's uncertainty. However, it works on a finite horizon setting, is restricted to unimodal state-transitions, and a particular shape of reward. PETS \cite{chua_deep_2018}, an improved version of PILCO, builds a probabilitstic model using a bootstrapped ensemble of neural-networks, and propagates the state-distribution using particles. This method, still requires a finite horizon. Furthermore, PETS does not make use of a parametrized policy, but instead a model predictive control. The controller requires multiple neural network evaluations, which can result in an issue when interacting with a real-time system. Our method, in contrast, works on the infinite-horizon setting, and the usage of a parametrized policy is more suitable for real-time operations. 

==> experiments/Cartpole_random.tex <==
\begin{figure}[t]
\begin{centering}
    \centering
    \includegraphics[scale=0.6]{figures/experiments/cartpole_randomwalk_samplesize.pdf}
    \caption[Returns in the Cartpole stabilization environment with randomly sampled data]{\textbf{Returns in the Cartpole stabilization environment with randomly sampled data} This plot compares the return obtained by NOPG and typical on- and off-policy algorithms in the CartPole task, as a function of the number of collected samples. NOPG's performance surpasses other algorithms by at least an order of magnitude. The TRPO and DDPG curves start at $5 \cdot 10^2$ samples because to accelerate training we only evaluate these algorithms after collecting every other $5 \cdot 10^2$ samples. The solid line represents the mean and the shaded area the 95\% confidence interval of 10 runs. The details used in this experiment are presented in \tabref{tab:cartpole_random_configs}.}

    \label{fig:cartpole_random}
\end{centering}
\end{figure}


==> experiments/Cartpole_real.tex <==
\begin{figure}[t]
\begin{centering}
    \centering
    \includegraphics[scale=0.5]{figures/experiments/cartpole_real.png}
    \caption[Evaluation of a policy optimized with NOPG-S in the real CartPole system]{\textbf{Evaluation of a policy optimized with NOPG-S in the real CartPole system} This stream of figures (left to right, top to bottom ordering) shows the application of a policy learned in simulation with NOPG-S in the real CartPole environment. The policy was trained using 1500 data points from trajectories with actions randomly sampled from a uniform distribution. Although a compliant policy can be learned with less samples, we found its actions alternated between very low and high signals, leading to very rough movements. We noticed that using more samples solved this problem.}
    \label{fig:cartpole_real}
\end{centering}
\end{figure}


==> experiments/Environments_schematics.tex <==
\begin{figure}[t]
\begin{centering}
    \begin{subfigure}{0.33\textwidth}
      \centering
      \includegraphics[scale=0.5]{figures/experiments/Pendulum_schematic.pdf}
      \caption{Pendulum}
      \label{fig:pendulum_schematic}
    \end{subfigure}%
    \begin{subfigure}{0.33\textwidth}
      \centering
      \includegraphics[scale=0.5]{figures/experiments/CartPole_schematic.pdf}
      \caption{CartPole}
      \label{fig:cartpole_schematic}
    \end{subfigure}
    \begin{subfigure}{0.33\textwidth}
      \centering
      \includegraphics[scale=0.5]{figures/experiments/MountainCar_schematic.pdf}
      \caption{MountainCar}
      \label{fig:mountaincar_schematic}
    \end{subfigure}    
    
    \caption[Environment schematics]{\textbf{Environment schematics} These figures depict the environments used in the experiments.}
    
    \label{fig:environment_schematics}
\end{centering}
\end{figure}

==> experiments/MountainCar_phase_portrait.tex <==
\begin{figure}[t]
\begin{centering}
    \begin{subfigure}{0.5\textwidth}
      \centering
      \includegraphics[scale=0.5]{figures/experiments/MountainCar_V_mu_0.pdf}
      \caption{Before any policy update}
      \label{fig:mountaincar_phase_portrait_a}
    \end{subfigure}%
    \begin{subfigure}{0.5\textwidth}
      \centering
      \includegraphics[scale=0.5]{figures/experiments/MountainCar_V_mu_251.pdf}
      \caption{After 251 policy updates}
      \label{fig:mountaincar_phase_portrait_b}
    \end{subfigure}
    
    \caption[Phase portrait of the value function and state distribution for the MountainCar experiment]{\textbf{Phase portrait of the value function and state distribution for the MountainCar experiment} The plots show the value function and state distribution estimates in the MountainCar environment using NOPG-D. The two leftmost plots show the estimates before any policy update and the rightmost after 251 updates. NOPG-D was trained with 4 trajectories provided by a human demonstrator with the details presented in \tabref{tab:mountaincar_configs}.}
    
    \label{fig:mountaincar_phase_portrait}
\end{centering}
\end{figure}


==> experiments/MountainCar_samplesize.tex <==
\begin{figure}[t]
\begin{centering}
    \centering
    \includegraphics[scale=0.6]{figures/experiments/mountaincar_samplesize.pdf}
    \caption[Returns in the MountainCar environment with varying number of trajectories]{\textbf{Returns in the MountainCar environment with varying number of trajectories} This plot shows the returns obtained by NOPG-D and NOPG-S as a function of the number of trajectories (roughly each trajectory corresponds to 450 samples). The human baseline corresponds to the average return in the human demonstrations and is depicted by the dashed line. The solid line represents the mean and the shaded area the 95\% confidence interval of 10 runs. The details used in this experiment are presented in \tabref{tab:mountaincar_configs}.}
    \label{fig:mountaincar_samplesize}
\end{centering}
\end{figure}


==> experiments/MountainCar_trajectory.tex <==
\begin{figure}[t]
\begin{centering}
    \centering
    \includegraphics[scale=0.6]{figures/experiments/MountainCar_trajectories.pdf}
    \caption[Trajectories in the state space of the MountainCar environment]{\textbf{Trajectories in the state space of the MountainCar environment} This figure shows two trajectories from evaluation runs of NOPG-D in the MountainCar environment. Trajectory's $1$ return is $-79$ and trajectory's $2$ is $-139$. The crosses denote the starting states and the circles the final states. The dashed vertical line at $x=-0.45$ depicts the goal state. The policy used was optimized with NOPG-D trained on 4 trajectories provided by a human demonstrator with the details presented in \tabref{tab:mountaincar_configs}.}
    \label{fig:mountaincar_trajectories}
\end{centering}
\end{figure}


==> experiments/Pendulum_phase_portrait.tex <==
\begin{figure}[t]
\begin{centering}
    \begin{subfigure}{0.5\textwidth}
      \centering
      \includegraphics[scale=0.5]{figures/experiments/Pendulum_V_mu_0.pdf}
      \caption{Before any policy update}
      \label{fig:pendulum_phase_portrait_a}
    \end{subfigure}%
    \begin{subfigure}{0.5\textwidth}
      \centering
      \includegraphics[scale=0.5]{figures/experiments/Pendulum_V_mu_301.pdf}
      \caption{After 301 policy updates}
      \label{fig:pendulum_phase_portrait_b}
    \end{subfigure}
    
    \caption[Phase portrait of the value function and state distribution for the Pendulum environment]{\textbf{Phase portrait of the value function and state distribution for the Pendulum environment} The plots show the value function and state distribution estimates in the Pendulum environment using NOPG-D, with a uniformly sampled data. The two leftmost plots show the estimates before any policy update and the rightmost after 301 updates. In this experiment, data was collected uniformly from a grid of state-action pairs (30 angles, 30 angular velocities, 2 actions) and NOPG-D trained with the details presented in \tabref{tab:pendulum_uniform_configs}.}
    
    \label{fig:pendulum_phase_portrait}
\end{centering}
\end{figure}


==> experiments/Pendulum_random.tex <==
\begin{figure}[t]
\begin{centering}
    \centering
    \includegraphics[scale=0.6]{figures/experiments/pendulum_randomwalk_samplesize.pdf}
    \caption[Returns in the Pendulum environment with randomly sampled data]{\textbf{Returns in the Pendulum environment with randomly sampled data} This plot compares the return obtained by NOPG and typical on- and off-policy algorithms in the Pendulum task, as a function of the number of collected samples. NOPG's performance surpasses other algorithms by at least an order of magnitude. The TRPO and DDPG curves start at $10^3$ samples because to accelerate training we only evaluate these algorithms after collecting every other $10^3$ samples. The solid line represents the mean and the shaded area the 95\% confidence interval of 10 runs. The details used in this experiment are presented in \tabref{tab:pendulum_random_configs}.}
    \label{fig:pendulum_random}
\end{centering}
\end{figure}


==> experiments/Pendulum_uniform.tex <==
\begin{figure}[t]
\begin{centering}
    \centering
    \includegraphics[scale=0.7]{figures/experiments/pendulum_uniform_samplesize.pdf}
    \caption[Returns in the Pendulum environment with uniform sampling]{\textbf{Returns in the Pendulum environment with uniform sampling} This box plot shows the return obtained by NOPG-D and NOPG-S as a function of the dataset size with samples from an uniform grid. The error bars show the results of 10 trials. The datasets' details are found in \tabref{tab:pendulum_uniform}.}
    \label{fig:pendulum_uniform}
\end{centering}
\end{figure}





==> experiments/Pendulum_uniform_table.tex <==
\begin{table}[ht]
\begin{center}
    \begin{tabular}{r r r}
        Sample size & NOPG-D & NOPG-S \\ \hline
        200  & $-3794.9 \pm 11.9$ & $-3788.5 \pm 00.9$  \\
        450  & $-576.3  \pm 03.1$  & $-594.1  \pm 39.8$ \\
        800  & $-572.3  \pm 02.3$  & $-572.8  \pm 03.9$ \\
        1250 & $-567.9  \pm 03.2$  & $-564.2  \pm 01.6$ \\
        1800 & $-472.0  \pm 28.8$  & $-457.9  \pm 26.0$ \\
        3200 & $-415.4  \pm 00.7$  & $-428.0  \pm 26.9$ \\
        \hline
    \end{tabular}
\end{center}

    \caption[Returns in the Pendulum environment with uniform sampling]{\textbf{Returns in the Pendulum environment with uniform sampling} This table presents the returns obtained by NOPG-D and NOPG-S as a function of the dataset size with samples from an uniform grid. Depicted are the mean and 95\% confidence intervals of 10 trials. The datasets' details are found in \tabref{tab:pendulum_uniform}.}
    \label{tab:pendulum_uniform_results}
\end{table}

